Attack of the Clones: Measuring the Maintainability, Originality and Security of Bitcoin 'Forks' in the Wild

Since Bitcoin appeared in 2009, over 6,000 different cryptocurrency projects have followed. The cryptocurrency world may be the only technology where a massive number of competitors offer similar services yet claim unique benefits, including scalability, fast transactions, and security. But are these projects really offering unique features and significant enhancements over their competitors? To answer this question, we conducted a large-scale empirical analysis of code maintenance activities, originality and security across 592 crypto projects. We found that about half of these projects have not been updated for the last six months; over two years, about three-quarters of them disappeared, or were reported as scams or inactive. We also investigated whether 11 security vulnerabilities patched in Bitcoin were also patched in other projects. We found that about 80% of 510 C-language-based cryptocurrency projects have at least one unpatched vulnerability, and the mean time taken to fix the vulnerability is 237.8 days. Among those 510 altcoins, we found that at least 157 altcoins are likely to have been forked from Bitcoin, about a third of them containing only slight changes from the Bitcoin version from which they were forked. As case studies, we did a deep dive into 20 altcoins (e.g., Litecoin, FujiCoin, and Feathercoin) similar to the version of Bitcoin used for the fork. About half of them did not make any technically meaningful change - failing to comply with the promises (e.g., about using Proof of Stake) made in their whitepapers.

==> Coin code similarity (Version 51646)/Makefile <==
#
# Makefile for acmart package
#
# This file is in public domain
#
# $Id: Makefile,v 1.10 2016/04/14 21:55:57 boris Exp $
#

PACKAGE=acmart


PDF = $(PACKAGE).pdf acmguide.pdf

all:  ${PDF} ALLSAMPLES


%.pdf:  %.dtx   $(PACKAGE).cls
	pdflatex $<
	- bibtex $*
	pdflatex $<
	- makeindex -s gind.ist -o $*.ind $*.idx
	- makeindex -s gglo.ist -o $*.gls $*.glo
	pdflatex $<
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $*.log) \
	do pdflatex $<; done


acmguide.pdf: $(PACKAGE).dtx $(PACKAGE).cls
	pdflatex -jobname acmguide $(PACKAGE).dtx
	- bibtex acmguide
	pdflatex -jobname acmguide $(PACKAGE).dtx
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' acmguide.log) \
	do pdflatex -jobname acmguide $(PACKAGE).dtx; done

%.cls:   %.ins %.dtx
	pdflatex $<


ALLSAMPLES:
	cd samples; pdflatex samples.ins; cd ..
	for texfile in samples/*.tex; do \
		pdffile=$${texfile%.tex}.pdf; \
		${MAKE} $$pdffile; \
	done

samples/%: %
	cp $^ samples


samples/$(PACKAGE).cls: $(PACKAGE).cls
samples/ACM-Reference-Format.bst: ACM-Reference-Format.bst

samples/%.pdf:  samples/%.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex-dev $(notdir $<); done

samples/sample-xelatex.pdf:  samples/sample-xelatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && xelatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && xelatex-dev $(notdir $<)
	cd $(dir $@) && xelatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && xelatex-dev $(notdir $<); done

samples/sample-lualatex.pdf:  samples/sample-lualatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && lualatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && lualatex-dev $(notdir $<)
	cd $(dir $@) && lualatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && lualatex-dev $(notdir $<); done



.PRECIOUS:  $(PACKAGE).cfg $(PACKAGE).cls

docclean:
	$(RM)  *.log *.aux \
	*.cfg *.glo *.idx *.toc \
	*.ilg *.ind *.out *.lof \
	*.lot *.bbl *.blg *.gls *.cut *.hd \
	*.dvi *.ps *.thm *.tgz *.zip *.rpi \
	samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst \
	samples/*.log samples/*.aux samples/*.out \
	samples/*.bbl samples/*.blg samples/*.cut 



clean: docclean
	$(RM)  $(PACKAGE).cls \
	samples/*.tex

distclean: clean
	$(RM)  *.pdf samples/sample-*.pdf

#
# Archive for the distribution. Includes typeset documentation
#
archive:  all clean
	COPYFILE_DISABLE=1 tar -C .. -czvf ../$(PACKAGE).tgz --exclude '*~' --exclude '*.tgz' --exclude '*.zip'  --exclude CVS --exclude '.git*' $(PACKAGE); mv ../$(PACKAGE).tgz .

zip:  all clean
	zip -r  $(PACKAGE).zip * -x '*~' -x '*.tgz' -x '*.zip' -x CVS -x 'CVS/*'

documents.zip: all docclean
	zip -r $@ acmart.pdf acmguide.pdf samples *.cls ACM-Reference-Format.*

.PHONY: all ALLSAMPLES docclean clean distclean archive zip


==> Coin code similarity (Version 51646)/sec/conclusion.tex <==
\section{Conclusion}
\label{sec:conclusion}

Many altcoins have been abandoned by their developers, or were outright scams from the start. Yet people continue to trade them, to use them, and even to invest in them. To investigate abuses that happen at scale, we also need analysis tools at scale. Therefore we built a semi-automated framework to inspect the maintenance and security of altcoins by analyzing their source code and project activities.

%The total market capitalization of suspicious altcoins seems substantial, but nobody has done a systematic study.

Our analyses indicate that many projects are not maintained properly or at all; that many leave known vulnerabilities unpatched; and that many do not even implement features promised in their whitepapers. About half of the 592 projects we inspected have not been updated during the last six months.  About a third of the projects forked from Bitcoin have 90\% or more code similarity with the Bitcoin version used to spawn them. Most concerning, over 80\% of 510 crypto projects we analyzed have at least one unpatched vulnerability. 

If the altcoin market is to become less of a lemons market, market participants need better ways of comparing project originality, liveness, and security. We believe that systematic code analysis reports are a necessary first step.



%\hl{We analyzed the correlations, respectively, between market capitalization and code maintenance activities ($r = 0.06$, p-value = 0.15), and between market capitalization and code similarity measured against Bitcoin ($r = 0.03$, p-value = 0.72), indicating that the cryptocurrency market may appear to be a classic lemon market.} To fix such a lemons market, market participants need better ways of comparing project originality, liveness, and security. We believe systematic code analysis reports are necessary first steps. Future work should include building verification tools to check whether features promised in whitepapers are indeed being implemented and added to projects. It should also include applying these techniques to other sectors of the software industries.

%We believe an efficient crypto project review and reporting service help investors and users make more informed decisions. Our framework can be extended for systematically reviewing crypto projects' code maintenance activities and security vulnerabilities, and producing consumer reports on the projects' originality, due diligence, and security. Such reports should be made available with free access (just like consumer reports for cars). This kind of ecosystem, in turn, would provide stronger motivations for crypto companies to make more honest claims about their products.



==> Coin code similarity (Version 51646)/sec/discussion.tex <==
\section{Discussion}
\label{sec:discuss}

\subsection{Is the cryptocurrency market a market for lemons?}
\label{subsec:How can we fix this}

There are strong financial incentives for individuals and companies to copy source code from existing crypto projects as they can launch a project quickly and cash in from an ICO. Many projects advertise fancy whitepapers without actually delivering promised features. Cohney et al.~\cite{cohney2019coin} found that smart contracts and ICO disclosures often do not match. Some popular ICOs have retained the power to modify their tokens' rights but did not disclose that ability in their whitepaper, which is consistent in our findings. We discovered some project teams (e.g., Block Array and Acoin) that focused on creating fancy whitepapers and websites rather than implementing promised features. Naive investors may be unable to distinguish such fly-by-night projects from well-maintained ones. 

To analyze the relationship between price and code quality, we computed Pearson's correlation coefficients between the market capitalization (i.e., price $\times$ the number of coins available) of crypto projects and their code maintenance activities, security, and code originality, respectively. The results show that there was no correlation between market capitalization and code maintenance activities ($r = 0.05$, p $=$ 0.44). Similarly, we failed to show correlation between market capitalization and the code similarity to Bitcoin ($r = 0.11$, p $=$ 0.29). However, the number of security vulnerabilities had a weak negative correlation with market capitalization ($r = -0.14$, p $<$ 0.05). These results indicate that altcoin code quality may not affect market prices: i.e., poor code quality does not necessarily mean that an altcoin is cheap, and vice versa. %These findings are consistent with the observations in a recent study~\cite{trockman2019striking} \hl{with 268 crypto projects, demonstrating that there is no compelling evidence for a dynamic relation between market capitalization and software metrics such as commits and lines of code changed.}

This suggests that the crypto market has turned into a classic ``market for lemons''~\cite{Akerlof70:lemon}: in the presence of asymmetric information and unconstrained opportunism, adverse selection can lead to inefficient markets where producers keep making low-quality products (lemons) instead of high-quality ones (peaches). In the crypto world, non-tech-savvy consumers will probably just read whitepapers and invest in a project without knowing how actively it is being maintained. The inevitable outcome is a crypto market full of scammy projects.

%inefficient and

%\hljs{We used the Pearson and Spearman's rank correlation analysis to evaluate the correlation between market capitalization and crypto originality or security. Interestingly, the Pearson correlation coefficient is 0.15 (0.001 p-value) and -0.11 (0.019 p-value) on the originality and security score, respectively. In addition, the Spearman's rank correlation coefficient is 0.17 (0.000 p-value) and -0.15 (0.002 p-value) on the originality and security score, respectively. There is a small relationship between the market capitalization and code quality (the originality or security scores of crypto projects).}

%We believe an efficient crypto project review and reporting service is necessary to bridge the information gap and help both investors and users make more informed decisions. 

%\hl{To help investors and users make more informed decisions, we can systemically produce consumer reports on the projects' originality, due diligence, and security using the proposed framework. Such reports should be made available with free access (just like consumer reports for cars). This, in turn, would provide stronger motivations for crypto companies to make more honest claims about their products.}

%, as well as the full analysis logs,

%As part of future work, an integral extension to be considered is a verification service that checks whether features promised in whitepapers are really being implemented.

\begin{comment}

\subsection{Maintenance, Security, and Originality}
\label{subsec:maintenance_discussion}

In Section~\ref{sec:results_maintenance}, we categorized 592 crypto projects into 2 groups by their code maintenance activities. In Section~\ref{sec:results_vulnerability}, we counted the number of vulnerabilities remaining in each of the XXX C-based crypto projects. In Section~\ref{sec:results_originality}, we computed the similarity scores between Bitcoin and its XXX descendants. Based on those results, we analyzed the relationships between code maintenance efforts, security, and code originality.

We examine the proportions of crypto projects with the number of vulnerabilities in each group categorized according to code maintenance activities by mapping XXX C-based crypto projects into clustering groups to analyze the relationship between code maintenance efforts and security.

% \begin{table}[!ht]
%     \centering
%     \caption{Proportion of crypto projects with the number of vulnerabilities in each group categorized according to code maintenance activities. Column `$\geq x$' refers to the number (proportion) of projects having at least $x$ vulnerabilities.}
%     \resizebox{0.86\linewidth}{!}{
%     \begin{tabular}{|c|c|c|c|c|c|}
%         \hline
%         ID & 0& $\geq 1$& $\geq 2$& $\geq 3$& $\geq 4$ \\\hline
%         %Number (\%) & 103 (19.9\%) & 415 (80.1\%) & 231 (44.6\%) & 138 (26.6\%) & 25 (4.8\%) \\\hline
%         1 & 28 (14.8\%) & 161 (85.2\%) & 100 (52.9\%) & 72 (38.1\%) & 10 (5.3\%) \\\hline
%         2 & 8 (22.2\%) & 28 (77.8\%) & 10 (27.8\%) & 0 (0.0\%) & 0 (0.0\%) \\\hline
%         3 & 15 (20.8\%) & 57 (79.2\%) & 35 (48.6\%) & 21 (29.1\%) & 7 (9.7\%) \\\hline
%         4 & 29 (30.5\%) & 66 (69.5\%) & 31 (32.6\%) & 21 (22.1\%) & 4 (4.2\%) \\\hline
%         5 & 5 (14.3\%) & 30 (85.7\%) & 16 (45.7\%) & 4 (11.4\%) & 0 (0.0\%) \\\hline
%         6 & 6 (10.7\%) & 50 (89.3\%) & 27 (48.2\%) & 12 (21.4\%) & 1 (1.8\%) \\\hline
%         7 & 12 (34.3\%) & 23 (65.7\%) & 12 (34.3\%) & 8 (22.9\%) & 3 (8.6\%) \\\hline
%     \end{tabular}}
%     \label{tab:maintain_cve}
% \end{table}

\begin{table}[!ht]
    \centering
    \caption{Proportion of crypto projects with the number of vulnerabilities in each group categorized according to code maintenance activities. Column `$\geq x$' refers to the number (proportion) of projects having at least $x$ vulnerabilities.}
    \resizebox{0.86\linewidth}{!}{
    \begin{tabular}{|c|c|c|c|c|c|}
        \hline
        ID & 0& $\geq 1$& $\geq 2$& $\geq 3$& $\geq 4$ \\\hline
        %Number (\%) & 103 (19.9\%) & 415 (80.1\%) & 231 (44.6\%) & 138 (26.6\%) & 25 (4.8\%) \\\hline
        1 & 43 (16.4\%) & 219 (83.6\%) & 135 (51.5\%) & 93 (35.5\%) & 17 (6.5\%) \\\hline
        2 & 60 (23.4\%) & 196 (76.6\%) & 96 (37.5\%) & 45 (17.6\%) & 8 (3.1\%) \\\hline
    \end{tabular}}
    \label{tab:maintain_cve}
\end{table}

% Table~\ref{tab:maintain_cve} shows that Cluster 7 (34.3\%) and Cluster 4 (30.5\%), compared to other clusters, contain greater number of projects without security vulnerability. On the other hand, a significant number of crypto projects in Cluster 1 (52.9\%), Cluster 3 (48.6\%), Cluster 6 (48.2\%), and Cluster 5 (45.7\%) have at least two security vulnerabilities. As one would expect, infrequently updated projects in Clusters 1, 3, and 6 are more likely to have vulnerabilities. Yet a significant number of frequently updated projects in Cluster 5 also have one or two unpatched security vulnerabilities.

% We examine the proportions of computed similarity scores in each of the 7 clusters to analyze the relationship between code maintenance and code originality.

Table~\ref{tab:maintain_cve} shows that Cluster 2 (23.4\%), compared to Cluster 1 (16.4\%), contain greater number of projects without security vulnerability. On the other hand, a significant number of crypto projects in Cluster 1 (51.5\%) has at least two security vulnerabilities. As one would expect, infrequently updated projects in Cluster 1 are more likely to have vulnerabilities. Yet a significant number of frequently updated projects in Cluster 2 also have one or two unpatched security vulnerabilities.


We examine the proportions of computed similarity scores in each of the 2 clusters to analyze the relationship between code maintenance and code originality.

% \begin{table}[!ht]
%     \centering
%     \caption{Proportion of crypto projects with the similarity scores in each group categorized according to code maintenance activities. Column `$\geq x\%$' refers to the number (proportion) of projects having a similarity score which is greater than or equal to $x\%$.}
%     \resizebox{0.86\linewidth}{!}{
%     \begin{tabular}{|c|c|c|c|c|c|}
%         \hline
%         ID & $<60\%$ & $\geq 60\%$ & $\geq 70\%$& $\geq 80\%$& $\geq 90\%$ \\\hline
%         %Number (\%) & 103 (19.9\%) & 415 (80.1\%) & 231 (44.6\%) & 138 (26.6\%) & 25 (4.8\%) \\\hline
%         1 & 9 (25.7\%) & 26 (74.3\%) & 24 (68.6\%) & 23 (65.7\%) & 21 (60.0\%) \\\hline
%         2 & 6 (17.1\%) & 29 (82.9\%) & 21 (60.0\%) & 19 (54.3\%) & 13 (37.1\%) \\\hline
%         3 & 5 (33.3\%) & 10 (66.7\%) & 8 (53.3\%) & 7 (46.7\%) & 6 (40.0\%) \\\hline
%         4 & 9 (56.3\%) & 7 (43.7\%) & 7 (43.7\%) & 6 (37.5\%) & 4 (25.0\%) \\\hline
%         5 & 23 (65.7\%) & 12 (34.3\%) & 7 (20.0\%) & 6 (17.1\%) & 5 (14.3\%) \\\hline
%         6 & 7 (38.9\%) & 11 (61.1\%) & 8 (44.4\%) & 7 (38.9\%) & 6 (33.3\%) \\\hline
%         7 & 3 (60.0\%) & 2 (40.0\%) & 1 (20.0\%) & 0 (0.0\%) & 0 (0.0\%) \\\hline
%     \end{tabular}}
%     \label{tab:origin_maintain}
% \end{table}


% Table~\ref{tab:origin_maintain} shows that a majority of crypto projects in Cluster 7 (60.0\%), Cluster 5 (65.7\%), and Cluster 4 (56.3\%) have similarity scores which are less than $60\%$. On the other hand, a majority of crypto projects in Cluster 1 (60.0\%) and Cluster 3 (40.0\%) have similarity scores greater than or equal to $90\%$. Based on those results, we carefully conclude that frequently updated projects are more likely to have lower similarity scores -- projects in Cluster 7, Cluster 5, and Cluster 4 have been frequently updated. In contrast, projects in Cluster 1 and Cluster 3 have rarely been updated. Interestingly, however, the projects in Cluster 2 show different characteristics: most of these projects have been updated frequently but also scored high in similarity scores.

Table~\ref{tab:origin_maintain} shows that a majority of crypto projects in Cluster 2 (44.0\%) have similarity scores which are less than $60\%$. On the other hand, a majority of crypto projects in Cluster 1 (54.0\%) have similarity scores greater than or equal to $90\%$. Based on those results, we carefully conclude that frequently updated projects are more likely to have lower similarity scores -- projects in Cluster 2 have been frequently updated. In contrast, projects in Cluster 1 have rarely been updated.

\begin{figure}[!ht]
\centering
\includegraphics[width=0.52\columnwidth]{fig/sim_vuln_plot.png}
\vspace{-0.2cm}
\caption{Scatter plot of similarity score versus the number of security vulnerabilities.}
\label{fig:sim_vuln_plot}
\end{figure}

We calculate the correlation coefficient between the similarity score and the number of security vulnerabilities for 157 Bitcoin descendent projects to analyze the relationship between security and code originality. Fig.~\ref{fig:sim_vuln_plot} is a scatter plot for code similarity scores and the number of security vulnerabilities. Unlike our expectation, there is an inverse correlation between code similarity score and number of security vulnerabilities (correlation coefficient is -0.25; and the p-value is less than 0.002). We found that a large number of cryptocurrencies were forked from a version of Bitcoin in which most vulnerabilities had already been fixed.



\subsection{Comparison with Reibel et al.'s work}
\label{sec: Comparison with Reibel}

%The purpose of this section is to clarify the differences between our work and theirs.

Reibel et al.~\cite{reibel2019short} investigated the code diversity of cryptocurrencies using their open-source code repositories. Because we also use open source code repositories for evaluating cryptocurrencies' originality and project maintenance, both approaches look similar in terms of code similarity analysis at first glance. However, there are two key differences between those approaches.

As discussed in Section~\ref{subsec:originality_method}, it may not be accurate to compare two crypto projects at one random point in time to assess the originality of a given altcoin (compared against its parent project) because the parent project can have a significant code update any time after code forking is complete. Therefore, the forked project's originality should be assessed by comparing it against the snapshot of the original parent project taken at the time of forking completion. For example, Reibel et al.'s method produces a similarity score of 24.1\% between Litecoin and Bitcoin despite the fact that the Litecoin source code is almost the same as the version of Bitcoin used for the fork. In contrast, we developed a technique to identify the forking point between a forked project and its parent project and compare the forked project with the snapshot of the original parent project taken at the time of forking. Our method produced a similarity score of 98.0\% between Litecoin and Bitcoin, demonstrating that our code similarity analysis (measuring the changes of forked projects over time) is more accurate than Reibel et al.'s method.

%Even though we improved the method to compare all Bitcoin versions, it outcomes 82.1\% of similarity and chooses the most similar Bitcoin version to June 2016, which has only 67 files in the commit. That is, if one-side of the being compared project has a tiny number of files, their method wrongly produces a high similarity score, and it is not correct similarity.

%it is not desirable to compare two crypto projects at one random point in time to assess the originality of an altcoin against its parent project because the parent project would be updated over time rather than the forked project. Therefore, we developed a technique to identify the forking point between a forked project and its parent project and compare the forked project with the snapshot of the original parent project taken at the time of forking. However, Reibel et al.'s approach just compared crypto projects at a specific point in time.

Moreover, to identify the extent to which cryptocurrencies reuse the source code of others, Reibel et al.~\cite{reibel2019short} suggested four simple heuristics such as name derivations, copyright derivations, common commits, and file derivations rather than computing the code similarity between crypto projects.

The name derivations method measured the Levenshtein distance~\cite{levenshtein1966binary} between cryptocurrencies' names (e.g., Bitcoin and Bitcoin Planet) to infer their forking relationship. However, according to our results in the code similarity analysis, this heuristic would likely lead to many false positives and negatives. For example, the code similarity score between Bitcoin and Bitcoin Scrypt is below 10\%. On the other hand, the code similarity score between Independent Money System and WomenCoin is 99.6\%.

The common commits\footnote{Reibel et al.~\cite{reibel2019short} named this approach ``Git forks.'' Unlike the name of the approach, however, they just checked whether cryptocurrencies have a common commit instead of actual fork relationships provided by GitHub. Therefore, we rename it ``common commits.''} method identified fork relationships with the information about commits that are contained in repositories. This approach first maps the commits to the lists of the repositories in which they appeared, and selects the oldest repository containing that commit as the original cryptocurrency and all other repositories in the list as its derivatives. However, this naive mapping might often guess fork relationships \emph{incorrectly}. For example, when crypto projects commonly contain a commit for a popularly used library, they can be wrongly identified as a forked project and its original cryptocurrency. To overcome this limitation, our approach checks whether two projects have all the same commits (i.e., common commit history) before the forking event rather than using a single common commit.

The copyright derivations method uses string matching in the copyright text (e.g., contributors of cryptocurrency-specific code) to identify potential derivatives based on the belief that most open source repositories make use of established libraries or other code. This approach might be useful for benign cryptocurrency developers who are not interested in concealing where their project is from. However, if someone intends to hide the original project information, the copyright information may be modified or deleted.

The file derivations method computes the hash of every source code file in two crypto projects. It then calculates a similarity score between them by dividing the number of files having the same hash value by the number of total files. However, this method has a clear limitation. If developers that reuse the codebase of an existing cryptocurrency commit minor changes to that code (e.g., coin names), the hash-based method would be useless. In practice, we encountered many such cases (e.g., replacements of ``bitcoin'' to ``acoin'' in Acoin) in our analysis results. To address this problem, we use \texttt{JPlag}~\cite{jplag,prechelt2002finding}, a well-known plagiarized code detection tool that is fairly robust against lexical alteration~\cite{ko2017coat}.

\end{comment}

%depends entirely on string matching in the copyright text, and 

%All of the above three methods simply check whether a cryptocurrency uses the codebase of another, but they do not measure the actual proportion of code that goes unmodified. To address this issue, Reibel et al.~\cite{reibel2018ravencoin} proposed the file derivations method. 


%$S_{hash}(C_{1},C_{2})$ between a cryptocurrency $C_{1}$ and another one $C_{2}$ where $A$ and $B$ are repositories of $C_{1}$ and $C_{2}$, respectively, as shown in Equation~\ref{eq:file}.

%\begin{small}
%\begin{equation} \label{eq:file}
%{S}_{hash}({C}_{1},{C}_{2})=\frac{\sum_{A\in {C}_{1}} {S}_{hash}(A,\bigcup_{B \in {C}_{2}}B)}{\sum_{A\in {C}_{1}}\#\ files\ in\ A}
%\end{equation}
%\end{small}

% \subsection{Threats to the study validity}
% \label{sec:threat}
\subsection{Limitations}
\label{sec:limit}

\textbf{Threats to validity.} %Our results may not generalize to all crypto projects. However, we evaluated our technique on large set of projects from the coinmarketcap website, which is widely recognized as the world's most-referenced website on active crypto projects. We, thus, believe that this selection significantly helps to ensure generalizability. To further improve external validity, we manually checked the validity of 20 crypto projects.
One threat to external validity is whether we used representative crypto projects for our study. A bias could have been introduced since we only analyzed C-language projects for vulnerability and originality. However, we note that most of the collected crypto projects, 86.3\%, have been developed in C/C++. A primary threat to internal validity is the bias that may have been introduced by researchers while conducting the case studies (see Section~\ref{subsec:Case studies}). We had to go through the whitepapers manually to identify altcoins that did not implement promised features (listed in the whitepapers). To minimize bias, the three researchers read the whitepapers separately, identified feature claims, and inspected the source code for compliance. After independently performing these analyses, the three researchers discussed their observations until they reached a consensus. A primary threat to construct validity is the metrics used in the study. To evaluate the crypto project maintenance quality, we used the 32 features available on GitHub. To evaluate their security, we examined patches implemented for known security vulnerabilities. To evaluate their originality, we measured the code similarity between the forked and original projects. We note that these metrics are just one of the few that can be used for evaluation, and more metrics might be studied in the future to improve the precision of our analysis.

% Our results may not generalize to all smart contracts or program types [67]. However, we evaluated our technique on a diverse set of contracts set of contracts from a wide range of domains. We, thus, believe that this selection significantly helps to ensure generalizability. To further improve external validity, we use publicly available benchmarks from related work [84].

%\noindent \textbf{Internal validity.} %Another potential issue has to do with whether systematic errors are introduced in the crawling the data of the crypto projects. When the crawling the data, 
%A primary threat to internal validity is the bias that may have been introduced by researchers while conducting the case studies (see Section~\ref{subsec:Case studies}). To identify altcoins that did not implement promised features (listed in the whitepapers), we had to go through the whitepapers manually. To minimize bias, the three researchers read the whitepapers separately, identified feature claims, and inspected the source code for compliance. After independently performing these analyses, the three researchers discussed their observations until they reached a consensus.

% Another potential issue has to do with whether systematic errors are introduced in the setup [67]. When comparing configurations, we always used the same seed inputs in order to avoid bias in the exploration.

%\noindent \textbf{Construct validity.} %Construct validity ensures that the evaluation measures what it claims. We compare several configurations of Harvey, and thus ensure that any improvements are exclusively due to techniques enabled in a given configuration.
%A primary threat to construct validity is the metrics used in the study. To evaluate the crypto project maintenance quality, we used the 32 features available on GitHub. To evaluate their security, we examined patches implemented for known security vulnerabilities. To evaluate their originality, we measured the code similarity between the forked and original projects. We note that these metrics are just one of the few that can be used for evaluation, and more metrics need to be studied in the future to improve analysis precision.

%alone might not be sufficient to measure crypto projects' maintenance, security, and originality fully.

% \subsection{Limitations}
% \label{sec:limit}

% \noindent \textbf{Biased dataset.} \hljs{We assumed that the C-based crypto projects are highly related to Bitcoin. }

\noindent \textbf{Determining forking points.} We developed two heuristics to guess the fork date of a given project (see Section~\ref{subsec:originality_method}). However, our methods can fail to estimate the exact forking time of a forked project, or to infer the forking relationship, when an old version of Bitcoin is used as new files to a repository instead of using the fork feature provided by GitHub. To tackle this issue, one might make comparisons with all past versions of the original project. %However, because comparisons with all past versions could be computationally expensive, we currently considered the past versions for the last six months only. %Therefore, we used heuristic techniques to reduce processing time. 

\noindent \textbf{Analyzing maintenance activities with Git messages.} When we analyze the maintenance activities on crypto projects, we only used the information obtained from Git. However, this information can be fabricated intentionally with dummy commits, dummy contributors, etc. We found that 22 projects in Cluster 4 are highly similar to their original projects (i.e., their similarity score is greater than or equal to 90\%) although they have been frequently updated. In such projects, we believe that developers may upload meaningless code periodically and add unnecessary comments so that their project appears to be on schedule and going well. We therefore suggest that further measurement techniques (including analysis of security vulnerabilities and code originality) should be developed as indicators of crypto project maintenance.

\begin{comment}
 
 (see Table~\ref{tab:origin_maintain})

\begin{table}[!ht]
    \centering
    \caption{Proportion of crypto projects with the similarity scores in each group categorized according to code maintenance activities. Column `$\geq x\%$' refers to the number (proportion) of projects having a similarity score which is greater than or equal to $x\%$.}
    \resizebox{0.86\linewidth}{!}{
    \begin{tabular}{|c|c|c|c|c|c|}
        \hline
        ID & $<60\%$ & $\geq 60\%$ & $\geq 70\%$& $\geq 80\%$& $\geq 90\%$ \\\hline
        1 & 14 (28.0\%) & 36 (72.0\%) & 32 (64.0\%) & 30 (60.0\%) & 27 (54.0\%) \\\hline
        2 & 48 (44.0\%) & 61 (56.0\%) & 44 (40.4\%) & 38 (34.9\%) & 28 (25.7\%) \\\hline
    \end{tabular}}
    \label{tab:origin_maintain}
\end{table}

\end{comment}

%\noindent \textbf{Limited dataset.} Because we only used C-based crypto projects for vulnerability and originality analyses, our analysis could be possibly impacted by the bias due to the limited projects. Therefore, our observations in vulnerability and originality analyses cannot be generalized for the projects in other programming languages. However, when we collected the crypto projects with the GitHub URL, the majority (80.7\%) of those projects have been developed in C language. Therefore, we focused on the analyses for C-based crypto projects.

%\noindent \textbf{Manual analysis of whitepaper contents.} The current version of the framework does not support automatic analysis of the features promised in whitepapers. After detecting code changes, we manually went through the whitepaper contents and investigated whether the code changes reflect promised features. Our future plans include automating this whitepaper verification process through text mining and machine learning techniques.

%\noindent \hljs{\textbf{Financial effects.} When the crypto projects had decided to stop developing their projects, it could be because of financial problems. Because of the crypto winter in 2018, lots of crypto projects had been disappeared}~\cite{whittemore, rocco}\hljs{. In the case of giving up the crypto projects because of the financial difficulty, the projects are hardly updated, and we might classify the projects to Cluster 1, 3, or 6. Therefore, we have a limitation about distinguishing between the failed projects and the ``lemon market.''}

%We analyzed source codes and white papers from 20 projects to investigate how much of the promised features have been implemented. Our findings indicate that many projects are not keeping their promises (and should be flagged) but we would need to investigate more projects as part of future work to further emphasize these scammy trends.

%For example,  We believe that some developers have intentionally introduced some unnecessary updates. 

% Construct validity ensures that the evaluation measures what it claims. We compare several configurations of Harvey, and thus, ensure that any improvements are exclusively due to techniques enabled in a given configuration.

==> Coin code similarity (Version 51646)/sec/framework.tex <==
\section{Evaluation framework}
\label{sec:methodology}

%To answer the research questions in Section~\ref{sec:research_questions}, 

We present a framework for (1) measuring the frequency of crypto project maintenance; (2) identifying security vulnerabilities, and investigating how quickly they are patched or not; and (3) measuring code similarity between crypto projects. Our analysis results are presented in Sections~\ref{sec:results_maintenance},~\ref{sec:results_vulnerability}, and~\ref{sec:results_originality}, respectively.

%Our framework is primarily designed to analyze developers' project maintenance activities, identify security vulnerabilities, and measure code similarity between Bitcoin and Bitcoin-forked projects. However, it can easily be extended to evaluate any crypto project by adjusting parameters (e.g., GitHub URLs). %Our framework uses Git repositories to collect the dataset for analyzing projects.

%We evaluated 643 crypto projects by downloading and inspecting their source code and commits. We used Git repositories to download such data -- the GitHub\footnote{\hl{GitHub is a Git repository hosting service. Source codes of a majority of crypto projects are published in GitHub.}} URLs for those cryptocurrencies were available on the CoinMarketCap website (\url{https://coinmarketcap.com/}).

\subsection{Code maintenance activities analysis}
\label{subsec:maintenance_method}

During the lifetime of any software project, maintenance is required to fix bugs and add new functionality. Crypto projects are no different. A number of metrics can be used to measure maintenance effort. 

% We do not have useful data on how much maintenance is required compared with other software classes. However, it is not zero, as can be seen from the constant activity by Bitcoin core developers.

We specifically used 32 features obtained from GitHub (for more details, see Appendix~\ref{sec: Features used for evaluating maintenance efforts}). These features can be categorized into three groups: (1) metrics for developers' engagement, (2) metrics for popularity, and (3) metrics for code updates. For the developers' engagement level, we use Commits, Branches, Releases, Contributors, Pull Requests, and Mean Developer Engagement (MDE)~\cite{adams2008detecting}. For project popularity, we analyze Watch, Star, Fork, Issues, Open Issues, and Closed Issues. Finally, for code update status, we use additions, deletions, and time intervals between commits. We use the mean and standard deviation values of these features over 3, 6, and 12 months to evaluate the code maintenance activities in the short-term, mid-term, and long-term, respectively. Although these metrics do not necessarily reflect software quality, Coleman et al.~\cite{Coleman94:software} demonstrated that quantitative metrics such as lines of code can be useful in evaluating software maintainability. Similarly, a recent study~\cite{Coelho20:Software} showed that such code commit-related attributes can be used to evaluate the maintenance level of open-source projects.

%\hljs{The metrics for developers' engagement directly influenced to measure the maintenance. A large number of commits mean a high possibility that the project is well-maintained.}

%\hljs{We assume that the popular projects try to be well-maintained because they have lots of interests.} 

%\hljs{The metrics for code updates are selected for confirming that the project is frequently updated in recent days.}

%To further characterize crypto projects, we categorize them into $k$ groups using the $k$-means clustering algorithm on the 32 features. After clustering, we analyze each group's characteristics and how many projects per group are still being developed actively. 

%This analysis is aimed at detecting poorly maintained projects.

\subsection{Security vulnerability analysis}
\label{subsec:vulernability_method}

In crypto projects, it is important to fix security vulnerabilities because of the direct risk of financial loss for users and investors. Therefore, we set out to identify which security vulnerabilities exist and how soon they are patched.

We examine source code for known vulnerabilities and note when each vulnerability is patched. It would be inefficient to download all previous versions of an altcoin's source code from its Git repository and check for vulnerable and patched code. We found that the total size of all previous versions of the crypto projects we analyzed is over 10.2 TB. We therefore developed a technique to inspect only source code changes available on GitHub for each code commit rather than looking at the full source -- we check whether deleted code contains a vulnerability or added code contains a patch. The process of our implementation is summarized in Appendix~\ref{appendix:Process of security vulnerability analysis}.

\subsection{Code similarity analysis}
\label{subsec:originality_method}

To detect and deter plagiarism -- heavy reuse of original code without adding new features -- we compare source code between projects to measure their similarity. If the source code of project $P_1$ has high similarity with that of project $P_2$, and $P_1$ was released after $P_2$, we assess whether a significant portion of $P_1$'s code has been reused without modification from $P_2$.

%\hljs{Ko et al.}~\cite{ko2017coat} \hljs{showed that JPlag achieved the best performance in various code changes among the code similarity measuring tools.} 

As most crypto projects are (hopefully) updated over time, it might not be accurate to compare two crypto projects at one random point in time to assess the originality of an altcoin against its parent project. Two projects could appear very different if the parent project underwent significant maintenance, even if the child had not. For example, the source code of Carboncoin, which was forked from Bitcoin on March 8th 2014, would be vastly different from the Bitcoin project snapshot taken on September 4th 2019 (33.5\%), even though Carboncoin has only been slightly updated. This is because Bitcoin has undergone significant maintenance over that five-year period. Therefore, the forked project's originality must be measured against a snapshot of the original parent project taken at the time of forking. We developed two heuristic methods to estimate the fork date of a given project based on the commits in Git. 

%Cryptocurrency developers do not usually disclose information about project forks, so 
%\noindent
\textbf{Heuristic 1:} If a project $P_\textnormal{forked}$ is forked from its original project $P_\textnormal{original}$ in Git, they would have the same code commit history before that forking event. However, their commit history is likely to be different from the time of the fork onward. Based on this intuition, we first determine whether a given crypto project $P_\textnormal{forked}$ is forked from another project $P_\textnormal{original}$, by checking whether the first few commits of the project $P_\textnormal{forked}$ are the same as the commits of the project $P_\textnormal{original}$. We then look for the first different commit history between the two projects and use that time as a forking point. 

%Finally, we download the source code of $P_\textnormal{original}$ at that time, which would be expected to be used for the fork. We note that the projects discovered by Heuristic 1 were clearly forked from $P_\textnormal{original}$ because their commit history is the same as that of $P_\textnormal{original}$, which can only be observed in forked repositories. 
%\noindent
\textbf{Heuristic 2:} We observed that some crypto projects were created by externally uploading source code files of another project. For those projects, we cannot use the first heuristic because we cannot compare common commits. In such cases, however, we can often observe the largest number of files being added or updated at a specific time to upload source code files of the parent project. Based on this intuition, in a given crypto project, $P_\textnormal{forked}$, we first identify which commit contains the largest number of file additions and/or changes from the project's commit. We use this commit time as a hypothetical (likely) forking point for project $P_\textnormal{forked}$ from its original project $P_\textnormal{original}$. We then sequentially compute the similarity between the source code of $P_\textnormal{forked}$ at the time of the fork and previous versions of source code of $P_\textnormal{original}$, respectively, before the time of the fork to find the most similar previous version of $P_\textnormal{original}$. This is because a crypto project can often be forked from an out-of-date version of its parent project. In principle, we need to examine all previous versions of $P_\textnormal{original}$ (before the time of the fork to find the source code version of $P_\textnormal{original}$) maximizing the similarity between $P_\textnormal{forked}$ and $P_\textnormal{original}$. However, to reduce computation cost, we only considered all previous versions for the last 6 months from the hypothetical (likely) forking point. Finally, if the computed similarity of the commit having the highest similarity score is greater than a predefined threshold, we assess that project $P_\textnormal{forked}$ was forked from project $P_\textnormal{original}$ with high probability. 

%We then treat the source code of $P_\textnormal{original}$ with the highest similarity score as the source code of $P_\textnormal{original}$.

%Appendix~\ref{appendix:Heuristic methods to measure the similarity between crypto projects} provides the details of our heuristic methods.

%\begin{figure}[!ht]
%\centering
%\includegraphics[scale=0.19]{fig/example_pastcompare.png}
%\vspace{-0.3cm}
%\caption{Example scenario where Carboncoin forked from Bitcoin reusing a significant portion of the source code in Bitcoin at the time of the fork.}
%\label{fig:pastexample}
%\end{figure}

%\begin{figure}[!ht]
%\centering
%\includegraphics[scale=0.3]{fig/scatter_plot.pdf}
%\vspace{-0.5cm}
%\caption{3d scatter example temp}
%\label{fig:3dscatter}
%\end{figure}

%(\url{https://github.com/carboncointrust/CarboncoinCore})

For a code-similarity scoring tool, we used \texttt{JPlag}~\cite{jplag,prechelt2002finding} because it has become known for its robustness against many of the techniques used to disguise similarities between plagiarized files~\cite{ko2017coat}. 

%supports repository-to-repository comparisons and 

%A high-level description of its operation is as follows~\cite{prechelt2002finding}: (1) \texttt{JPlag} removes comments, variable names, function names, and whitespaces; (2) it converts the source code into string tokens; and (3) token strings are compared to measure similarity using the Greedy String Tiling algorithm~\cite{wise1993string}.

\subsection{Dataset}
\label{subsec:dataset}

%we collected 643 crypto projects (see the list of those projects in \url{https://bit.ly/3A0ppjl}) with their GitHub URL from 1,578 cryptocurrencies registered on CoinMarketCap~\cite{coinmarketcap}.

For evaluation, we initially collected all 1,627 crypto projects registered on CoinMarketCap~\cite{coinmarketcap} as of July 2018. However, because we were only interested in cryptocurrency projects that operate independently on their own blockchains, we did not include token projects (e.g., ERC-20, ERC-223, and ERC-721 types) in our analysis. Finally, we selected 592 crypto projects\footnote{The list is online at \url{https://bit.ly/3A0ppjl}.} that were registered as an independent blockchain platform, and for which the official GitHub URLs were available. We started from the list of registered cryptocurrencies on July 22nd, 2018 but downloaded the latest version before September 3rd, 2019 of their source code files. Since our goal was to study the long-term (1--2 years) project development and maintenance activities and trends of cryptocurrency projects, we selected projects that were created around 2018 and analyzed their historical data for the following 1--2 years. Further, we needed ground-truth information about the survivability of the projects (i.e., whether projects were eventually reported as scams, or inactive, or were still operating) to investigate the relationship between projects' maintenance activities and some form of ground truth about project survivability.

%-- again, implying that it is necessary to choose projects that have some historical data as well as project active state information available.


%The only way we can collect labeled ground truth information about the project long-term survivability (i.e., whether a project has been delisted from CoinMarketCap, or reported as a scam project, or its GitHub URL has been removed) is to analyze projects’ long-term past data.

%All GitHub URLs of the crypto projects were obtained from the CoinMarketCap website, widely recognized as the top source for trading information on active crypto projects. If a project's source code was not available via the CoinMarketCap website, we excluded it from our study as we wanted to check the authenticity of each project's source code in an automated manner. Additionally, we only considered crypto projects available on the GitHub platform to avoid biases due to differences in platforms' features. %\hljs{For example, a crypto project, named OKB, does not provide any source code link at CoinMarketCap.} \hljs{For example, a crypto project, named Cardano, provides the source code link but it is not GitHub-related URL.}

%\footnote{\hl{GitHub is a Git repository hosting service. The source code of a majority of crypto projects is published in GitHub.}}

%\footnote{\url{https://coinmarketcap.com/historical/20180722/}}

%For example, We excluded the token projects which resident on the Ethereum blockchain.

%The C-based crypto projects have 1,206.1 files on average (with a standard deviation of 2,832.0 files), and the average lines of code of the files is 163,901.7 (with a standard deviation of 388,063.9).

%Therefore, if a project contains source code files having the file extension of `\texttt{c}', `\texttt{h}', `\texttt{cpp}', or `\texttt{hpp}', we simply regarded the project as a C-based project. Based on this categorization, we collected 519 C-based crypto projects.

%However, we only used 518 C-based altcoins for the security vulnerability analysis because of the structured way information about Bitcoin vulnerabilities is provided. Finally, we analyzed the code similarity between 519 projects only written in C language for the code similarity analysis. However, we used all 643 projects because maintenance may not be highly related to the underlying programming language.

Crypto projects are implemented in a wide variety of programming languages including C, Go, Python, and Java. However, we found that 511 (86.3\%) of the 592 crypto projects we obtained from our selection process are written in C/C++. Because the archetypal crypto project -- Bitcoin -- is written in C/C++, we focused on C-based crypto projects for our vulnerability and code similarity analyses. For the code maintenance analysis, we used all 592 projects because maintenance may not be highly related to the underlying programming language.

%because maintenance may not be highly related to the underlying programming language. 

%However, we only used 518 C-based altcoins for the security vulnerability analysis because of the structured way information about Bitcoin vulnerabilities is provided. Finally, we analyzed the code similarity between 519 projects only written in C language for the code similarity analysis. 

%We gathered pairs of vulnerable and patched code for 11 Bitcoin CVEs from the commits in Bitcoin (see the list of CVEs in \url{https://bit.ly/2D4Ropl}).%\stjs{. The detailed CVE information is summarized in Appendix}~\ref{appendx:CVE}.

==> Coin code similarity (Version 51646)/sec/introduction.tex <==
\section{Introduction}
\label{sec:intro}

%Following the success of Bitcoin~\cite{bitcoin}, thousands of open-source cryptocurrency projects emerged. Entrepreneurs launching a new cryptocurrency (or ``altcoin'') typically claim to tackle existing coins' drawbacks. For example, ``Dash''~\cite{dash} appeared in January 2014 to make transactions harder to trace through its Coinjoin protocol~\cite{coinjoin}; ``Zcash''~\cite{sasson2014zerocash} was introduced in October 2016 to further protect user anonymity by re-mining coins; and ``Bitcoin Cash'' emerged in August 2017 to improve the transaction throughput of Bitcoin by increasing the block size. 

%Following the success of Bitcoin~\cite{bitcoin}, thousands of open-source cryptocurrency projects emerged. Entrepreneurs launching a new cryptocurrency (or ``altcoin'') typically claim to tackle existing coins' drawbacks. 

As of 2021, over 6,000 cryptocurrencies are available for trading on the market~\cite{coinmarketcap} and have attracted attention from securities regulators. However, many cryptocurrency projects (hereinafter referred to as {\em crypto projects}) stopped their development~\cite{rocco,whittemore} and rarely introduce any code updates~\cite{zetzsche2017ico}. A 2018 article in the Wall Street Jurnal claimed that 16\% of 3,291 initial coin offering (ICO) projects show signs of plagiarism, identity theft and promises of improbable goals~\cite{wallstreet}. Worse yet, according to Deadcoins~\cite{deadcoins} and Coinopsy~\cite{coinopsy}, about 1,000 different crypto projects have failed to meet their goals~\cite{scamcoin}. There seems to be little motivation for companies to implement the promised features after their ICO, or to fix security vulnerabilities quickly, because it is not easy for regular investors to validate the claimed features or announced updates by examining the code commits in their project repositories.

%In fact, many crypto projects stopped developing because of their financial problems~\cite{rocco,whittemore}.

%The cryptocurrency world may be the only technology where so many competitors offer similar services yet claiming unique benefits, including scalability, fast transactions, and security. But are these projects really offering unique features and significant enhancements over their competitors? %Are they patching known security vulnerabilities in a timely manner? Are investors making informed decisions?



%The market for altcoins would appear to be a classic ``market for lemons''~\cite{Akerlof70:lemon} in that investors lack information about crypto projects' code originality, maintenance, and security, and have to rely on marketing material such as whitepapers on project websites.

%\footnote{These reports are useful but rely on users' self-reported feedback.}

%These reports are useful but rely on users' self-reported feedback. There is a lack of assessment tools or processes for systematically analyzing crypto projects' due diligence at the code maintenance level.

In this paper, we claim that (1) many commercially traded crypto projects are not being appropriately maintained, leave known vulnerabilities unpatched, or do not implement promised features, and (2) to improve market transparency and reliability, it is necessary to provide an automated method and tool to regularly assess projects' originality, liveness and security. 

We developed a framework to collect crypto projects' code and project information and analyze the code maintenance liveness, originality, and security. Our framework and dataset will help facilitate more efficient and precise analyses of emerging crypto projects. Our contributions are summarized below:

%Our framework is capable of (1) inspecting developers' code maintenance activities, (2) measuring security vulnerabilities and patch implementation delays, and (3) measuring source code similarities between crypto projects to evaluate their code originality.

%\hljs{Notably, the information asymmetry makes lemons in crowdfunding via the internet}~\cite{ibrahim2015equity} \hljs{. Even though most of the projects' code is publicly opened, the market for altcoins is the market that the investors are regarded it hard to understand paradoxically.} 

%Where irresponsible or inactive projects are done at scale, countermeasures must also scale to be effective. To achieve this goal, we have developed a code inspection framework (\url{https://github.com/Anony-temp/Attack-of-the-Clones}). Our framework is capable of (1) inspecting developers' code maintenance activities, (2) measuring security vulnerabilities and patch implementation delays, and (3) measuring source code similarities between crypto projects to evaluate their code originality. These analyses are possible because most crypto projects have made their source code available online. %through GitHub.

%For market transparency and reliability, it is necessary to provide some means to assess project originality, liveness, and security. 

%we conduct large-scale analyses to identify inactive and insecure altcoins across 643 crypto projects. We present comprehensive code analysis results as the first step toward providing the originality and security information about crypto projects to the public. 

%Recently, Reibel et al.~\cite{reibel2018ravencoin} suggested the use of project information (e.g., cryptocurrency name, common commit, copyright, and identical files) to detect code reuse among crypto projects. However, their heuristics cannot detect \emph{hidden} forking relationships because they rely merely on the project information or hashes of files, which can be easily modified if developers intentionally try to hide forking relationships. To overcome this limitation, we developed a code similarity analysis tool that finds hidden forking relationships between crypto projects and compares their source codes while being fairly robust against lexical alteration.

%Using this framework, we conducted a large-scale empirical study to evaluate code maintainability, originality, and security of 643 crypto projects that can be tracked in CoinMarketCap~\cite{coinmarketcap}. We demonstrate that many popularly traded crypto projects are not being appropriately maintained, leave known vulnerabilities unpatched, or do not implement promised features. Our key observations are as follows:

\begin{itemize}
    \item We collected 592 crypto projects and analyzed their code maintenance data. We found that 288 crypto projects (48.6\%) have not been updated at all for the last six months, and about three-quarters of these disappeared, or were reported as scams or inactive at the end of two years (see Section~\ref{sec:results_maintenance}). %A lack of maintenance activity can indicate that a project is a scam or has simply been abandoned. 
    \item We conducted a study of security patches in Bitcoin derivatives with over 1.6 million code commits. We developed a code analysis tool to identify security vulnerabilities in projects' Git repositories, and the times at which they were patched. For 11 vulnerabilities patched in Bitcoin, over 80\% of the projects we studied still leave at least one unpatched. The {\em mean time to patch} is 237.8 days (see Section~\ref{sec:results_vulnerability}). %For example, the seven-year-old vulnerability (CVE-2013-4627) still exists in 56.8\% of them. Outdated, vulnerable third-party libraries are also widely used: a messaging library bug (CVE-2019-6250) that can be leveraged to run arbitrary code is prevalent in 22.2\% of the projects (see Section~\ref{sec:results_vulnerability}).%The use of outdated third-party libraries containing serious bugs such as  CVE-2014-0224 (34.4\%)~\cite{cve-2014-0224}, CVE-2014-0160 (29.2\%)~\cite{cve-2014-0160}, and CVE-2019-6250 (22.2\%)~\cite{cve-2019-6250} is also a problem.
    \item We evaluated forked projects' originality compared to their parent project. Our results show that over a third of the 157 altcoins that are likely to have been forked from Bitcoin still have 90\% or more code similarity with the Bitcoin version used to spawn them. We did a deep dive into 20 altcoins that are very similar to a Bitcoin version, discovering that about half of them do not contain any technically meaningful update and fail to comply with technical promises -- including about tokenization and Proof of Stakes (PoS) -- made through their whitepapers (see Section~\ref{sec:results_originality}).
    %do not contain any significant changes, and 6 of them did not implement the features such as tokenization and Proof of Stakes (PoS) promised in their white papers.
%    \item We found that the cryptocurrency market may appear to be a classic ``market for lemons''~\cite{Akerlof70:lemon} based on the correlation analysis between market capitalization and code maintenance activities ($r = 0.06$, p-value = 0.15), and between market capitalization and code similarity measured against Bitcoin ($r = 0.03$, p-value = 0.72), indicating that cryptocurrency market prices may not necessarily reflect on the code quality (see Section~\ref{subsec:How can we fix this}). 
\end{itemize}

%The proposed framework can be used to facilitate separation of \emph{crypto lemons} in the market -- projects that are unoriginal, vulnerable, or both -- to help investors assess financial and security risks better .

%The rest of this paper is organized as follows. Section~\ref{sec:research_questions} provides our research motivations and research questions. Section~\ref{sec:methodology} describes our analysis methodology to evaluate cryptocurrency projects. Section~\ref{sec:results_originality}, \ref{sec:results_maintenance}, and \ref{sec:results_vulnerability} present the originality, maintenance efforts, and software vulnerability measurement results, respectively, for the existing 643 cryptocurrency projects. Section~\ref{sec:discuss} discusses the key issues and limitations of our evaluation method. Related work is covered in Section~\ref{sec:related}. Finally, our conclusions are in Section~\ref{sec:conclusion}.

==> Coin code similarity (Version 51646)/sec/related_work.tex <==
\section{Related work}
\label{sec:related}

%Our discussion of related work is grouped as follows.

% We treat as related research that measures either general properties of open-source software, or research that measures properties of cryptocurrencies. In terms of the former, there have been numerous papers measuring GitHub reopsitories. For example, Hu et al. and Thung et al. measured the influence of software projects according to their position of their repositories and developers in the GitHub social graph, and others have taken advantage of the volume of source code available on GitHub to analyze common coding practices or how bugs vary across different programming languages.

\noindent
\textbf{Understanding the landscape of cryptocurrencies.}
As cryptocurrencies became popular, we have seen a broader academic interest in the activities associated with blockchains such as user privacy~\cite{Biryukov14:bitcoin,Goldfeder18:bitcoin}, market manipulation~\cite{xu2019anatomy}, money laundering~\cite{brenig2015economic,barone2019cryptocurrency}, network availability~\cite{vasek2014empirical}, bug characteristics~\cite{wan2017bug}, and scams~\cite{vasek2015there,vasek2018analyzing}. Zetzsche et al.~\cite{zetzsche2017ico} showed that many ICOs have utterly inadequate information disclosure; e.g., more than half of ICO whitepapers are silent on the initiators. Oliva et al.~\cite{oliva2020exploratory} conducted a study of smart contracts in the Ethereum platform and found that only a small number (0.05\%) of the smart contracts were actively used in most (80\%) of the transactions that were sent to contracts. Trockman et al.~\cite{trockman2019striking} investigated if there is a dynamic relation between software metrics and market capitalization for 268 cryptocurrencies using dynamic regression models and found that there was no compelling evidence of a relationship. Lucchini et al.~\cite{Lucchini04:cryptocurrency} found that the number of developers working on a cryptocurrency project correlates positively with its market capitalization. This paper further analyzed correlation coefficients between market capitalization and code maintenance activities, unpatched security vulnerabilities, and code similarity, respectively. Reibel et al.~\cite{reibel2019short} analyzed the code diversity of cryptocurrencies' open-source code repositories. Their study is similar to ours in some ways because both exploit project information extracted from repositories to evaluate the originality of crypto projects. However, their approach relied on rather naive rules (name derivations, copyright derivations, common commits, and file derivations) that often misinterpret the relationships between crypto projects. In addition to offering a more thorough code-diversity analysis, we analyze security vulnerabilities and measure how much Bitcoin's descendent projects differ from Bitcoin. 

%We highlight key differences between Reibel et al.'s approach and ours in Section~\ref{sec: Comparison with Reibel}.

%,Heilman15:bitcoin,Apostolaki17

%This project attempts to directly estimate the activities, maintenance, as well as security of altcoins purely based on the public code repositories, and as a result, aims to seamlessly scale to future altcoin projects without human assistance. 

\noindent
\textbf{Evaluating the quality of project management.} Many techniques have been proposed to evaluate the quality of open-source projects. Thung et al.~\cite{thung2013network} constructed social graphs between projects to identify which were influential by
using PageRank on the graph. Hu et al.~\cite{hu2016influence} also measured the importance
of software repositories using social-network analysis techniques. In those studies, social graphs between projects were constructed by using project information explicitly provided by Git, such as common developers between projects or star relationships.  Unlike their work, our proposal can identify hidden fork relationships between projects because we assume that some developers may intentionally cover up a fork relationship. Coelho et al.~\cite{Coelho20:Software} proposed a method to evaluate the maintenance of open-source projects using classification algorithms and 13 features such as the number of commits in the last time interval and the maximum number of days without commits in the last time interval. We extended their analysis method with 19 additional features such as commit time interval and MDE value to evaluate crypto project maintenance activities.

%\hljs{They used 13 features for evaluating crypto projects. We also used the features they used and the additional features such as the commit time interval, MDE value, and so on, which are useful in evaluating the crypto projects (see Fig.}~\ref{fig:features}\hljs{).} \stjs{We also used several commit-related features to evaluate the level of maintenance activities of crypto projects.}


%The studies focused on the connection between the GitHub projects, and also the ramifications of the projects. However, the cryptocurrencies might be similar to each other because they are built upon the blockchain scheme. 

%kamiya2002ccfinder, 

\noindent
\textbf{Detecting known vulnerabilities.} Several proposals (e.g., \cite{jiang2007deckard,sajnani2016sourcerercc,perl2015vccfinder}) have been introduced for detecting similar vulnerabilities in code bases. However, their detailed inspection techniques are too time-consuming for mass measurement. The total number of commits analyzed in our experiments is over 1.6 million. Our study's precondition -- identifying bugs introduced by the parent project (e.g., Bitcoin) in a child project (e.g., Litecoin) -- makes our evaluation tractable even without detailed inspection techniques. Li et al.~\cite{li2017large} collected security patches using Git commits and conducted a large-scale empirical study of them. However, unlike Li et al.'s work~\cite{li2017large}, we identified the locations of those vulnerabilities and patches in Bitcoin derivatives using their source code as well as Git commits because we wanted to also cover the cases where patch information is not reported through Git commits. Hum et al.~\cite{hum2020coinwatch} used clone-code detection to find vulnerable crypto projects, and discovered 786 vulnerabilities from 384 projects using 4 CVEs (CVE-2018-17144, CVE-2016-10724, CVE-2016-10725, and CVE-2019-7167). In this paper, we report a much more efficient vulnerable code detection method: we use code commits to inspect code changes only, rather than examining the full source code. This enabled us to cover all previous versions of crypto projects and identify when security vulnerabilities were patched. We also used 11 CVEs -- CVE-2018-17144 is only common CVE between Hum et al.'s work and ours.

%More sophisticated vulnerability detection techniques might work technically for evaluating the security of altcoins. However, the precondition of our study --- identifying bugs introduced by the parent project (e.g., Bitcoin) in a child project (e.g., Litecoin) --- makes our evaluation tractable even without such sophisticated techniques. We note that the technique called VulDeePecker~\cite{li2018vuldeepecker} would be useful in locating similar types of bugs among altcoins. 

%The state-of-the-art vulnerability detection methodology includes deep learning~\cite{li2018vuldeepecker}. Such techniques might work technically for evaluating the security of altcoins. However, the precondition of our study --- identifying bugs introduced by the parent project (e.g., Bitcoin) in a child project (e.g., Litecoin) --- makes our evaluation tractable even without such sophisticated techniques. We note that the technique called VulDeePecker~\cite{li2018vuldeepecker} would be useful in locating similar types of bugs among altcoins. However, in mass measurement, such detailed inspection takes a long time. We note that the total number of commits analyzed in our experiments is over 1.6 million. We may have slightly reduced the correctness of vulnerability detection, but have significantly increased the coverage of the inspection. \hljs{In the large-scale study of the open-source projects}~\cite{li2017large}\hljs{, they estimated vulnerabilities and patches on the project using the public vulnerability information in detail. However, we tried to invest the tendency of security of altcoins about Bitcoin-related vulnerabilities.}

%\noindent
%\textbf{Measuring code similarity.} We opted to use a widely used code plagiarism tool called \texttt{JPlag}~\cite{jplag} because \texttt{JPlag} uses programming language syntax and program structure to detect plagiarized codes and hence is robust against many kinds of attempts to disguise similarities between plagiarized files~\cite{ko2017coat}. However, there have been several proposals to improve performance where similarity calculation is a critical element of the use cases (e.g., real-time clone detection, searching a massive number of projects, etc.) Such techniques (e.g., using a Bloom filter in ReDeBug~\cite{jang2012redebug} or hashing scheme of VUDDY~\cite{kim2017vuddy}) could be adopted in our project if the number of altcoins increases. 


%As also used source codes, Hu et al.~\cite{hu2016influence} and Thung et al.~\cite{thung2013network} measured the open-source projects using GitHub properties such as a social graph, volume, and so on. The general open-source analysis is not enough to analyze the cryptocurrency projects because they share a lot of properties by frequent forking.

%Vasek et al.~\cite{vasek2015there} presented the empirical analysis of Bitcoin-based scams. 

% [37]\hljs{There is no citation number 37.}/\cite{ron2013quantitative} in \cite{reibel2018ravencoin}.
% look interesting:
% - Network structure of social coding in GitHub.
% - Patterns of folder use and project popularity: A case study of GitHub repositories
% - GitHub repository health report. \url{https://github.com/pelson/repohealth.info}


% Connecting blockchains, interledger, sidechains and cross-blockchain Technologies

% Our study builds on prior work in software reliability growth and on efforts to characterize the social utility of finding and reporting vulnerabilities. We have applied models that define software reliability in terms of the number of faults in a body of code. Such models “apply statistical techniques to the observed failures during software testing and operation to forecast the product’s reliability” [2, p. 6]. As faults are identified and removed, the system will fail less frequently and hence be more reliable. These models can thus be utilized to estimate characteristics about the number of faults remaining in the system and when those faults may cause failures. These estimates can be then be used to gauge the amount of further testing required to meet reliability requirements. Eric Rescorla first applied reliability growth models to post-release vulnerability reporting data in order to question the social utility of publicly disclosing vulnerabilities [11]. He found no clear trend reduction in the rate of vulnerability reporting, and he estimates that the half-life of a vulnerability is between 10 months and 3.5 years. However, the ICAT database he uses is not focused on vulnerability age, and it does not reliably report the dates on which vulnerabilities were born.6 For our analysis, we used the version control system to ascertain the exact date of birth for each vulnerability in our data set. Furthermore, we test more models (seven) than the two that he evaluated. In addition, we only present results from the model that passed both goodness-of-fit and one-stepahead predictive accuracy tests; Rescorla only utilized the former test. Another related body of literature looks at measuring software security through market-mechanisms. L. Jean Camp and Catherine Wolfram proposed a market through which vulnerability credits could be traded; such markets have worked previously to create incentives for the reduction of negative externalities like environmental pollutants [3].

% \hl{In the first paragraph, we need to present previous studies to measure the quality of open source projects.}
% \hl{The information available from an open source repository can also be examined when evaluating the maintenance quality of an open source project}~\cite{MI1,najm2014measuring,spinellis2009evaluating}. 

% \hl{In the second paragraph, we need to introduce several projects to evaluate cryptocurrencies.}

% \hl{In the third paragraph, we need to present previous methods to compute the similarity between codes.}



%When measuring similarities between cryptocurrencies, we also used several similarity calculation tools, or code plagiarism detection tools, other than the fuzzy hash algorithm. In this section, we briefly mention the tools that we have used and how these tools operate to detect similar parts of the code.
% \subsection{maintenance efforts index}
% \label{subsec:mi}
%There are many research about evaluating open source project using maintainability index. Samoladas et al ~\cite{samoladas2004open} examined five active open source code using MI and monitored the quality of projects. Kaur et al ~\cite{kaur2011determination} proposed maintainability index using package (MIP) that exploit MI for measuring quality of object oriented system. The Maintainability Index (MI) was proposed by Oman. It is a metric consisting of Line of Code, Halstead Volume and Cyclomatic Complexity. It indicates that how this project is well maintained and high MI implies good maintainability. Halstead Volume is used for measuring software complexity. It is calculated by number of operands and operators. Cyclomatic Complexity was given by McCabe and also used for measuring complexity of source code. Drawing control flow graph of program, it is produced by number of edges and node in the graph. 


% \subsection{Cryptocurrency evaluating report}
%Weiss Crypto Ratings announced report about cryptocurrency evaluating ~\cite{weiss}. 122 Cryptocurrencies are evaluated based on technology, adoption, risk and reward. But there is no detail description to evaluate cryptocurrencies in report. The report describes the views and trends of the overall cryptocurrency. Among 4 models, focusing technology and adoption, Bitcoin got A and Etherum got A-.  China's Center for Information and Industry Development (CCID) also announced cryptocurrency ranking ~\cite{ccid}. CCID evaluated 35 cryptocurrencies based on three models: basic technology, applicability and creativity. This ranking shows that EOS ranks 1st and Ethereum ranks 3rd and differently with Weiss Crypto Ratings, Bitcoin ranks 15th. CCID also doesn't explain ranking methodology in detail. It seems that Weiss Crypto Ratings and CCID results are driven subjectively by human experts.


%%\subsection{JPlag}
%%\label{subsec:jplag}

%%JPlag~\cite{prechelt2002finding}, which is a plagiarism detecting tool written in Java, was used during our cryptocurrency similarities measurement. The tool is able to compare two source codes which are written in various languages, including Java, C, Python, Scheme and C\#. Given a directory, JPlag calculates similarity percentages for all possible pairs of repositories in the directory. The tool outputs the similarity percentages in standard output but also provides HTML files to allow the users analyze more thoroughly. The HTML files display some of the matches sorted by average similarity and the matches sorted by maximum similarity. The average similarity gives the average of coverages of both programs being compared. The maximum similarity gives the maximum of coverages of both programs being compared, and this is meaningful if the two programs being compared are vastly different in size. JPlag measures the similarity by changing the program into token strings first and using "Greedy String Tiling"~\cite{wise1993string} to compare the token strings. 
%%
%% JPlag is used for detecting software source code plagiarism.[] JPlag can find renaming variables, functions or split/merge of variable declarations and ignore comments, blank lines and constant values. The algorithm that JPlag use is "Greedy String Tiling" that compare two token strings. JPlag split number of lines to several tokens. Two token sets A and B is compared using algorithm. JPlag supports Java, Python, Pascal, C, C++ and normal strings.
%%



%%\subsection{SIM}
%%\label{subsec:sim}

%% SIM was written by Dick Grune, vrije university, Amsterdam. SIM makes string to tokens in each source code and compare each token of code. SIM shows similarity between two source codes and similar parts visually. SIM provides execution program for each languages. SIM supports C++, Java Pascal, Miranda , Assembler code and arbitrary text. 

%%We also used SIM which is another plagiarism detection tool that works on C, Java, Pascal, Modula-2, Lisp, Miranda, 8086 assembler code or text files. The tool is both available in C sources and MSDOS binaries. Unlike JPlag, SIM does not support directory to directory comparisons, and only displays similarity percentages between files. Therefore, to come up with a similarity percentage between two cryptocurrency repositories, we used the method that we mentioned in Section~\ref{subsec:originality}. SIM converts all units in the input files into tokens then uses these tokens to calculate a similarity percentage.


==> Coin code similarity (Version 51646)/sec/research_question.tex <==
\section{Research questions}
\label{sec:research_questions}
%This paper has been motivated by the following three research questions. %\hljs{This paper has been motivated by evaluating the crypto projects ecosystem with the following three research questions.}

The market for altcoins appears to be a classic ``market for lemons''~\cite{Akerlof70:lemon} in that investors lack information about crypto projects' code originality, maintenance, and security, and have to rely on marketing material such as whitepapers on project websites. There is little motivation for companies to implement promised features honestly or quickly patch security vulnerabilities since investors have no easy way of checking their development activities or verifying whether updates claimed on websites or social media are indeed being committed to code repositories. This paper aims to facilitate the identification of potential \emph{crypto lemons} in the market -- projects that are unoriginal, vulnerable, or both -- to help investors assess financial and security risks better. We focus on the following three research questions to achieve this goal:

%\textbf{RQ1: \hl{How many crypto projects have persistently been maintained in source code?}}

\textbf{RQ1: Are crypto projects updating their source code?}

One way to assess the liveness and credibility of a crypto project is to investigate its code maintenance activities. To answer RQ1, we designed an evaluation framework that automatically analyzes a project's source code and commits to its code repository.

%\textbf{\hl{RQ2: How many crypto projects have  been updated for security patches in a timely manner?}}

\textbf{RQ2: Are crypto projects implementing security patches in a timely manner?}

To evaluate the security of crypto projects, we analyze how quickly known security vulnerabilities have been patched. To answer RQ2, we identify vulnerable code fragments in crypto projects and investigate when these code fragments were patched. According to Gartner's report~\cite{gartner}, about 90\% of successful Internet-based attacks that exploited software applications have not been patched properly. Therefore, if a crypto project ignores vulnerabilities or patches slowly, this indicates high-security risks.

\textbf{RQ3: Are crypto projects forked from Bitcoin making significant code changes to the original code?}

%More than 2,000 different altcoins have been launched since July 2011 to address inadequacies (e.g., transaction throughput, latency, or anonymity) in existing cryptocurrencies such as Bitcoin. 

To answer RQ3, we investigate whether these altcoins have indeed made meaningful enhancements from their original parent projects (e.g., by implementing the features promised in their whitepapers). We do not claim that the code similarity measurement alone is sufficient to identify scam or inactive projects. However, the code similarity measurement examines whether forked projects have been sufficiently modified from the original Bitcoin code over time to justify their establishment as a new blockchain product. 

%For this analysis, we focus on Bitcoin-forked projects, as Bitcoin is the most widely adopted cryptocurrency and has the biggest market capitalization.



==> Coin code similarity (Version 51646)/sec/results_CVE.tex <==
\section{Security vulnerability analysis}
\label{sec:results_vulnerability}

This section presents the results of our security vulnerability analysis, which used the method described in Section~\ref{subsec:vulernability_method}. To gauge whether crypto project maintainers mitigate security vulnerabilities in a timely manner, we examined whether Bitcoin's known vulnerabilities were patched in 510 other C-based crypto projects. We first considered all known 39 Bitcoin CVEs since 2011\footnote{The Bitcoin CVEs before 2011 are not related to other crypto projects because the first altcoin was launched in the middle of 2011.}. However, we were only able to obtain code information about 11 CVEs from the Bitcoin Git messages (see the detailed information about those CVEs in Appendix~\ref{appendix:CVE}). For each of these CVEs, we got source code versions for before and after CVE occurrence, which enabled us to extract vulnerable codes and patched/fixed codes based on diff results. We manually verified the correctness of those codes. Appendix~\ref{appendix:Vulnerable and patched code fragment for CVE-2013-4627} shows an example of vulnerable and patched code fragments for ``CVE-2013-4627.'' 

%\footnote{We collected 511 C-based crypto projects in total and excluded Bitcoin itself from the comparison.}

\begin{table}[!ht]
\vspace{-0.6cm}
    \centering
    \caption{Proportion of vulnerable crypto projects.}
    \resizebox{0.56\linewidth}{!}{
    \begin{tabular}{|c|c|c|r|}
        \hline
        CVE ID & Type & CVSS & \multicolumn{1}{c|}{Number (\%)} \\\hline
        CVE-2012-1909 & DoS & 5.0 & 0 (0.0\%) \\\hline
        CVE-2012-3789 & DoS & 5.0 & 0 (0.0\%) \\\hline
        CVE-2012-1910 & DoS, Execute code & 7.5 & 0 (0.0\%) \\\hline
        CVE-2012-2459 & DoS & 5.0 & 0 (0.0\%) \\\hline
        CVE-2014-0160 & Overflow, Gain information & 5.0 & 149 (29.2\%) \\\hline
        CVE-2013-4627 & DoS & 5.0 & 294 (57.7\%) \\\hline
        CVE-2013-4165 & Gain information & 4.3 & 43 (8.4\%) \\\hline
        CVE-2014-0224 & Gain information & 5.8 & 176 (34.5\%) \\\hline
        CVE-2018-12356 & Execute code & 7.5 & 0 (0.0\%) \\\hline
        CVE-2018-17144 & DoS & 5.0 & 27 (5.3\%) \\\hline
        CVE-2019-6250 & Execute code, Overflow & 9.0 & 113 (22.2\%) \\\hline
    \end{tabular}}
    \label{tab:patch results}
\vspace{-0.5cm}
\end{table}

We determined whether 11 vulnerabilities were appropriately patched in each project based on such code fragment pairs. These results are summarized in Table~\ref{tab:patch results}, indicating that a significant number crypto projects leave some vulnerabilities unpatched. 294 (57.7\%) of cryptocurrencies are vulnerable to CVE-2013-4627~\cite{cve-2013-4627}, which has a Common Vulnerability Scoring System (CVSS)\footnote{CVSS provides a numerical (0-10) representation of the severity of an information security vulnerability.} score of 5.0. Thus, in many crypto projects, the memory of blockchain nodes can be exhausted with intentionally created dummy transactions. 176 (34.5\%) cryptocurrencies are vulnerable to CVE-2014-0224~\cite{cve-2014-0224}, named ``CCS Injection,'' that has a CVSS score of 5.8. This vulnerability originates from OpenSSL (\url{https://www.openssl.org/}), the most widely used open-source cryptographic library. This vulnerability allows attackers to carry out man-in-the-middle attacks for hijacking sessions and stealing sensitive information via a specially crafted TLS handshake. The impact of this vulnerability may be rather limited in crypto projects because SSL/TLS protocols are not directly used as communication protocols in most implementations. However, this shows that the code maintainaance -- and perhaps the security awareness level -- of a significant number of cryptocurrencies is poor because the patched OpenSSL version was released in June 2014. In the case of Bitcoin, this bug was immediately fixed by upgrading the OpenSSL library. 

As for real security risks, 149 crypto projects (29.2\%) are vulnerable to ``Heartbleed,'' CVE-2014-0160~\cite{cve-2014-0160}, which has a CVSS score of 5.0. As with CVE-2014-0224~\cite{cve-2014-0224}, this vulnerability originates from OpenSSL. 113 (22.2\%) are vulnerable to CVE-2019-6250~\cite{cve-2019-6250} that has a CVSS score of 9.0. This vulnerability originates from ZeroMQ libzmq (also known as 0MQ) (\url{https://github.com/zeromq/libzmq}), which is a library for high-performance asynchronous messaging. This vulnerability might be critical for some projects because a successful exploit could allow an attacker to overwrite an arbitrary amount of bytes beyond the bounds of a buffer, which, in turn, could be leveraged to run arbitrary code on a target system. The presence of these vulnerabilities demonstrates that a significant number of crypto projects are at actual risk of cyber-attacks; and people are investing in them without being aware of material security risks.



% CVE ID & Type~\footnote{\url{https://www.cvedetails.com/vulnerabilities-by-types.php}} & CVSS & Number (\%) \\\hline

%\hljs{Even though the vulnerabilities affect the project under specific circumstances, they have potential dangers in the future.} 

We note that the most serious vulnerabilities, namely CVE-2014-0224~\cite{cve-2014-0224}, CVE-2014-0160~\cite{cve-2014-0160}, and CVE-2019-6250~\cite{cve-2019-6250}, are vulnerabilities in third-party libraries imported into crypto projects. Given that the use of third-party libraries has become a common practice in the cryptocurrency industry, it is essential to keep them up to date. It is well known that they often contain serious bugs~\cite{Watanabe17:software}.

Table~\ref{tab:patch results} shows that no crypto projects containing the vulnerabilities (CVE-2012-1909~\cite{cve-2012-1909}, CVE-2012-3789~\cite{cve-2012-3789}, CVE-2012-1910~\cite{cve-2012-1910}, and CVE-2012-2459~\cite{cve-2012-2459}) which were discovered in 2012. We surmise that the reason for these results is that all but 24 of the projects we studied were forked after June 2012.

\begin{table}[t]
\centering
\caption{Proportion of inactive/scam crypto projects with the number of vulnerabilities.}
%\caption{Proportion of inactive crypto projects with the number of vulnerabilities. Row `$\geq x$' refers to the number (proportion) of crypto projects having at least $x$ vulnerabilities.}
\label{table:delist_cve}
\resizebox{0.85\linewidth}{!}{
\begin{tabular}{|c|r|r|r|r|r|r|}
\hline
\# vuln. & \multicolumn{1}{c|}{Number (\%)} & \multicolumn{1}{c|}{N/A in CoinMarketCap} & \multicolumn{1}{c|}{N/A in GitHub} & \multicolumn{1}{c|}{Coinopsy} & \multicolumn{1}{c|}{Deadcoins} & \multicolumn{1}{c|}{All} \\\hline
0        &  99 (19.4\%) &  40 (40.4\%) & 5 (5.1\%) & 28 (28.3\%) & 17 (17.2\%) & 54 (54.5\%) \\\hline
$\geq 1$ & 411 (80.6\%) & 211 (51.3\%) & 8 (1.9\%) & 104 (25.3\%) & 64 (15.6\%) & 262 (63.7\%) \\\hline
$\geq 2$ & 227 (44.5\%) & 124 (54.6\%) & 5 (2.2\%) & 68 (30.0\%) & 36 (15.9\%) & 154 (67.8\%) \\\hline
$\geq 3$ & 138 (27.1\%) &  81 (58.7\%) & 1 (0.7\%) & 42 (30.4\%) & 23 (16.7\%) & 98 (71.0\%) \\\hline
$\geq 4$ &  25 (4.9\%)  &  19 (76.0\%) & 0 (0.0\%) & 7 (28.0\%) & 7 (28.0\%) & 21 (84.0\%)\\\hline
All      & 510 (100.0\%) & 251 (49.2\%) & 13 (2.5\%) & 132 (25.9\%) & 81 (15.9\%) & 316 (62.0\%) \\\hline
\end{tabular}}
\vspace{-0.5cm}
\end{table}

We also counted the number of vulnerabilities remaining in each crypto project. Table~\ref{table:delist_cve} lists the number of security vulnerabilities remaining for each of the 510 C-based projects, showing that 411 out of 510 (80.6\%) have at least one unpatched vulnerability.

To analyze whether the survivability of those altcoins was correlated with the number of vulnerabilities, we analyzed the proportion of inactive/scam projects with the number of vulnerabilities in the manner described in Section~\ref{sec:results_maintenance}. The results are presented in Table~\ref{table:delist_cve}, indicating that the number of vulnerabilities does indeed seem related to survivability. 84.0\% of altcoins with 4 or more vulnerabilities disappeared from the market or were reported as scams or inactive, while this fate befell only 54.5\% of those with no vulnerability.

To analyze the time it took for the altcoin developers to fix each of the 11 vulnerabilities, we computed the elapsed time between (a) when Bitcoin first released a patch, and (b) when altcoins applied that patch on their code. Fig.~\ref{fig:patch_days} shows the median and mean values of the elapsed time, which were 16 and 237.8 days (with a standard deviation of 453.6 days). The large gap between median and mean values indicates that about half the vulnerabilities were patched quickly -- 56.6\% were patched within 16 days of the corresponding patch being applied to Bitcoin -- whereas the other half took weeks, months, or even years before they were fixed. 

\begin{figure}[!ht]
\vspace{-0.3cm}
\centering
\includegraphics[trim={0 0.1cm 0 0.8cm},clip, width=0.58\linewidth]{fig/patch_days.pdf}
\vspace{-0.4cm}
\caption{Number of days taken to fix a vulnerability.}
\label{fig:patch_days}
\vspace{-0.5cm}
\end{figure}

To explore the relationship between code maintenance activities and unpatched  vulnerabilities, we compared the number of vulnerabilities remaining in each project between Clusters 1, 2, 3 and 4. In Cluster 1, the median and mean values are 2.0 and 1.80 (with a standard deviation of 1.20); in Cluster 2, the median and mean values are 1.5 and 1.73 (with a standard deviation of 1.30); in Cluster 3, the median and mean values are 1.0 and 1.28 (with ta standard deviation of 1.09); in Cluster 4, the median and mean values are 1.0 and 1.60 (with a standard deviation of 0.98). There is a statistically significant difference between the four clusters (p $<$ 0.0002, Kruskal-Wallis test).

%we compared the time taken to patch security vulnerabilities between Cluster 1, 2, 3, and 4, which were obtained in Section~\ref{sec:results_maintenance}. In Cluster 1 \hl{(10.0\% patch ratio)}, the median, and mean values are 188 and 277.5 days (with the standard deviation of 298.4 days), respectively; in Cluster 2 \hl{(11.7\% patch ratio)}, the median and mean values are 1.5 and 354.6 days (with the standard deviation of 595.7 days), respectively; in Cluster 3 \hl{(15.8\% patch ratio)}, the median and mean values are 12 and 391.3 days (with the standard deviation of 598.0 days), respectively; in Cluster 4 \hl{(32.5\% patch ratio)}, the median and mean values are 7 and 188.1 days (with the standard deviation of 449.8 days), respectively. There is a statistically significant difference between the four clusters (p $<$ 0.0001, Kruskal-Wallis test). Similarly, 



\begin{comment}

\noindent \fbox{\begin{minipage}{\linewidth}
\hljs{55.7\% were patched on the same day as the corresponding patch was applied to Bitcoin (\textbf{RQ2}). On the other hand, the other half took weeks, months, or even years until they were fixed.}
\end{minipage}}

\end{comment}


%These findings are consistent with the observations in a recent study~\cite{li2017large} with general open source projects, demonstrating that it takes a long time, sometimes multiple years, for a vulnerability to be patched after the initial report.

==> Coin code similarity (Version 51646)/sec/results_maintenance.tex <==
\section{Code maintenance activity analysis}
\label{sec:results_maintenance}

This section presents the results of code maintenance activity analysis, which was performed using the method described in Section~\ref{subsec:maintenance_method}. We used the $k$-means clustering algorithm to categorize 592 crypto projects into $k$ groups by code maintenance activity to detect poorly maintained or inactive code development. In our dataset, the best clustering results were obtained when $k=4$ (see Appendix~\ref{appendix:Selection of k in k-means clustering}). The clustering results are summarized in Table~\ref{table:Clustering results of cryptocurrencies by code maintenance activities}.

\begin{table}[!ht]
\vspace{-0.7cm}
    \centering
    \caption{Clustering results of cryptocurrencies by code maintenance activity during 2018. Examples are selected by market capitalization.}
    \resizebox{0.74\linewidth}{!}{
        \begin{tabular}{|c|c|c|c|}
            \hline
            ID & \# & Examples & Properties \\ \hline
            1 & 207 & DGB, LSK, XZC, LBC, GAP & rarely updated during the last 12 months\\ \hline
            2 & 81 & RDD, FST, TTC, MOON, SUMO & rarely updated during the last 6 months\\ \hline
            3 & 61 & XEM, SC, PZM, UNO, SLS & rarely updated during the last 3 months\\ \hline
            4 & 243 & BTC, ETH, XRP, LTC, ADA & frequently updated during all periods\\ \hline
        \end{tabular}}
    \label{table:Clustering results of cryptocurrencies by code maintenance activities}
\vspace{-0.5cm}
\end{table}

We identified the clustering results' key attributes using the best-first search algorithm~\cite{pearl1984intelligent}. Fig.~\ref{fig:features} shows the comparison results of clusters for those key attributes (e.g., number of added lines of code, time interval between commits), indicating that the projects in Cluster 4 were persistently maintained well over time while the projects in Cluster 1, 2, and 3 were rarely updated for the last 12, 6, and 3 months, respectively. Surprisingly, 288 out of 592 (48.6\%) crypto projects (included in Cluster 1 and 2) have not been updated at all during the last six months, revealing that about half of crypto projects have been poorly maintained or abandoned.

%We then compared the statistics (e.g., the number of projects delisted from CoinMarketCap) between the clusters identified from the code maintenance activities.

% This section presents the results of code maintenance activity analysis, which was performed using the method described in Section~\ref{subsec:maintenance_method}. We \hl{aimed to categorize} 915 crypto projects into several meaningful groups by their code maintenance efforts to detect poorly maintained or inactive code development. We extracted 23 features related to code maintenance activities from each project, and we used those features and the $k$-means clustering algorithm to categorize the projects into $k$ groups. We then compared the statistics (e.g., the number of projects that were delisted from CoinMarketCap) between the clusters identified from the code maintenance activities. --- New Experiments (915: C/C++, Total: 1,480), (570: C/C++, Latest: 904)

%Appendix~\ref{appendix:Silhouette coefficient analysis} shows the silhouette coefficient of clustering results.

%\footnote{The coefficient combines the average within-cluster distance with the average nearest-cluster distance to assign a value between -1 and 1. A value below zero denotes that the observation is probably in the wrong cluster, and a value closer to 1 denotes that the observation is a great fit for the cluster and clearly separated from other clusters.}

%\begin{figure}[t]
%\begin{center}
%\begin{tabular}{c}
%\includegraphics[trim={0 0.3cm 0 0},clip, scale=0.16]{fig/Silhouette_all.pdf} %
%\end{tabular}
%\end{center}
%\vspace{-0.6cm}
%\caption{Silhouette results from $k=2$ to $20$.}
%\label{fig:silhouette}
%\end{figure}

% Even though the $k$-means clustering algorithm produced the best silhouette value when $k = 2$, we realized that two clusters are not sufficient to categorize inattentively (inactively maintained) projects from diligently maintained projects in a fine-grained manner. Therefore, we set $k = 7$, leading to clustering results that produced the second-best silhouette value. The clustering results are summarized in Table~\ref{table:Clustering results of cryptocurrencies by code maintenance activities}. We identified the key attributes of the clustering results using the best first search algorithm~\cite{pearl1984intelligent} as a feature selection method. Fig.~\ref{fig:features} shows the comparison results of clusters for those key attributes (e.g., number of contributors, number of forks, the time interval between commits, number of commits in the last time interval, etc.). We note that such code commits related attributes can be used to evaluate the maintenance level of open-source projects according to a recent study~\cite{Coelho20:Software}. 


\begin{figure}[!ht]
    \vspace{-0.2cm}
    \centering
    \begin{minipage}[b]{0.31\textwidth}
        \centering 
        \includegraphics[width=\textwidth]{fig/boxplot_X3M_ave_updated.pdf}
    \end{minipage}\hfill
    \begin{minipage}[b]{0.31\textwidth}
        \centering 
        \includegraphics[width=\textwidth]{fig/boxplot_X3M_std_updated.pdf}
    \end{minipage}\hfill
    \begin{minipage}[b]{0.31\textwidth}
        \centering 
        \includegraphics[width=\textwidth]{fig/boxplot_X6M_ave_additions.pdf}
    \end{minipage}\vfill
    \begin{minipage}[b]{0.31\textwidth}
        \centering \includegraphics[width=\linewidth]{fig/boxplot_X6M_std_updated.pdf}
    \end{minipage}\hfill
    \begin{minipage}[b]{0.31\textwidth}
        \centering \includegraphics[width=\linewidth]{fig/boxplot_X12M_ave_additions.pdf}
    \end{minipage}\hfill
    \begin{minipage}[b]{0.31\textwidth}
        \centering \includegraphics[width=\linewidth]{fig/boxplot_X12M_ave_updated.pdf}
    \end{minipage}\hspace{2em}\\ 
    \vspace{-0.2cm}
    \caption{Properties of each cluster in the top 6 key attributes (mean time interval between commits for 3M (M stands for months.), standard deviation time interval between commits for 3M, mean additions for 6M, standard deviation time interval between commits for 6M, mean additions for 12M, and mean time interval between commits for 12M). To better visualize the results, we exclude some outliers in analyzing mean additions for 6M and 12M.}
    \label{fig:features}
    \vspace{-0.2cm}
\end{figure}

%To analyze the health status of each cluster, we additionally calculated the proportion of scam or inactive crypto projects in each cluster based on the reports from CoinCodeCap~\cite{coincodecap}, Deadcoins~\cite{deadcoins}, and Coinopsy~\cite{coinopsy}. The results are presented in Table~\ref{table:badcoinlist}.

To show the relevance of the clustering results, we compared the survivability of each cluster with the proportion of projects that disappeared from the market or were reported as a scam or inactive. We regard a project as inactive if it is not listed on CoinMarketCap, or its GitHub URL is unavailable (in September 2021). Note that a crypto project can only be listed on CoinMarketCap if it is available on a public exchange service and has a non-zero trading volume. Also, we regard a project as a scam if it is listed on Deadcoins~\cite{deadcoins} or Coinopsy~\cite{coinopsy}. The survivability results are presented in Table~\ref{tab:disappear_coins}, indicating that most crypto projects (59.1\%) disappeared from the market, or were reported as scams or inactive in just two years. Furthermore, it seems that the code update activities could be used as a signal for project survivability -- the cluster of frequently-updated crypto projects (in Cluster 4) has the lowest proportion (38.3\%) of inactive projects while the crypto projects in Cluster 1 (76.8\%), Cluster 2 (74.1\%), and Cluster 3 (62.3\%) that were rarely updated are highly like to be inactive or scams.

\begin{table}[t]
\vspace{-0.3cm}
    \centering
    \caption{Proportion of inactive/scam crypto projects in each cluster.}
    \resizebox{0.85\linewidth}{!}{
    \begin{tabular}{|c|r|r|r|r|r|r|}
        \hline
        ID & \multicolumn{1}{c|}{Number (\%)} & \multicolumn{1}{c|}{N/A in CoinMarketCap} & \multicolumn{1}{c|}{N/A in GitHub} & \multicolumn{1}{c|}{Coinopsy} & \multicolumn{1}{c|}{Deadcoins} & \multicolumn{1}{c|}{All} \\\hline
        %Number (\%) & 103 (19.9\%) & 415 (80.1\%) & 231 (44.6\%) & 138 (26.6\%) & 25 (4.8\%) \\\hline
        1 & 207 (35.0\%) & 131 (63.3\%) & 7 (3.4\%) & 75 (36.2\%) & 30 (14.5\%) & 159 (76.8\%) \\\hline
        2 & 81 (13.7\%) & 52 (64.2\%) & 5 (6.2\%) & 18 (22.2\%) & 14 (17.3\%) & 60 (74.1\%) \\\hline
        3 & 61 (10.3\%) & 27 (44.3\%) & 3 (4.9\%) & 14 (23.0\%) & 15 (24.6\%) & 38 (62.3\%) \\\hline
        4 & 243 (41.0\%)& 70 (28.8\%) & 2 (0.8\%) & 35 (14.4\%) & 26 (10.7\%) & 93 (38.3\%) \\\hline
        All & 592 (100.0\%) & 280 (47.3\%) & 17 (2.9\%) & 142 (24.0\%) & 85 (14.4\%) & 350 (59.1\%) \\\hline
    \end{tabular}}
    \label{tab:disappear_coins}
    \vspace{-0.4cm}
\end{table}

\begin{comment}

\begin{table}[t]
\vspace{-0.3cm}
    \centering
    \caption{Proportion of inactive/scam crypto projects in each cluster.}
    \resizebox{0.77\linewidth}{!}{
    \begin{tabular}{|c|c|c|c|c|c|c|c|}
        \hline
        ID & \# & N/A in CoinMarketCap & N/A in GitHub & Coinopsy & Deadcoins & CoinCodeCap & All \\\hline
        %Number (\%) & 103 (19.9\%) & 415 (80.1\%) & 231 (44.6\%) & 138 (26.6\%) & 25 (4.8\%) \\\hline
        1 & 81 & 52 (64.2\%) & 5 (6.2\%) & 18 (22.2\%) & 14 (17.3\%) & 36 (44.4\%) & 72 (88.9\%) \\\hline
        2 & 207 & 131 (63.3\%) & 7 (3.4\%) & 75 (36.2\%) & 30 (14.5\%) & 62 (30.0\%) & 176 (85.0\%) \\\hline
        3 & 243 & 70 (28.8\%) & 2 (0.8\%) & 35 (14.4\%) & 26 (10.7\%) & 49 (20.2\%) & 116 (47.7\%) \\\hline
        4 & 61 & 27 (44.3\%) & 3 (4.9\%) & 14 (23.0\%) & 15 (24.6\%) & 23 (37.7\%) & 45 (73.8\%) \\\hline
        All & 592 & 280 (47.3\%) & 17 (2.9\%) & 142 (24.0\%) & 85 (14.4\%) & 170 (28.7\%) & 409 (69.1\%) \\\hline
    \end{tabular}}
    \label{tab:disappear_coins_coincodecap}
    \vspace{-0.6cm}
\end{table}
\end{comment}

% \begin{table}[!ht]
%     \centering
%     \caption{Proportion of inactive crypto projects in each cluster in May 2021.}
%     \resizebox{0.85\linewidth}{!}{
%     \begin{tabular}{|c|c|c|c|c|}
%         \hline
%         ID & \# & N/A in CoinMarketCap & N/A in GitHub & All \\\hline
%         %Number (\%) & 103 (19.9\%) & 415 (80.1\%) & 231 (44.6\%) & 138 (26.6\%) & 25 (4.8\%) \\\hline
%         1 & 288 & 174 (60.4\%) & 10 (3.5\%) & 178 (61.8\%) \\\hline
%         2 & 355 & 96 (27.0\%) & 7 (2.0\%) & 98 (27.6\%) \\\hline
%     \end{tabular}}
%     \label{tab:disappear_coins_2021}
% \end{table}
%\vspace{-0.2cm}
% \begin{table}[t]
%     \centering
%     \caption{Proportion of scam or inactive cryptocurrencies in each cluster.}
%     \resizebox{0.52\linewidth}{!}{
%         \begin{tabular}{|c|c|c|c|c|}
%             \hline
%             ID & \# & Coinopsy & Deadcoins & All\\ \hline
%             1 & 81 & 18 (22.2\%) & 14 (17.3\%) & 24 (29.6\%) \\\hline
%             2 & 207 & 75 (36.2\%) & 30 (14.5\%) & 86 (41.5\%) \\\hline
%             3 & 243 & 35 (14.4\%) & 26 (10.7\%) & 46 (18.9\%) \\\hline
%             3 & 61 & 14 (23.0\%) & 15 (24.6\%) & 21 (34.4\%) \\\hline
%             All & 592 & 142 (24.0\%) & 85 (14.4\%) & 177 (29.9\%) \\\hline
%         \end{tabular}
%     }
%     \label{table:badcoinlist}
%     \vspace{-0.5cm}
% \end{table}
%\vspace{-0.5cm}
% \begin{table}[!ht]
%     \centering
%     \caption{Proportion of scam or inactive cryptocurrencies in each cluster in May 2021. \hl{CoinCodeCap result is not available in 2021 because the website disappeared.}}
%     \resizebox{0.65\linewidth}{!}{
%         \begin{tabular}{|c|c|c|c|c|c|}
%             \hline
%             ID & \# & CoinCodeCap & Deadcoins & Coinopsy & All\\ \hline
%             1 & 288 & -- & 54 (18.8\%) & 84 (29.2\%) & 115 (39.9\%)\\ \hline
%             2 & 355 & -- & 67 (18.9\%) & 52 (14.6\%) & 91 (25.6\%)\\ \hline
%             All & 643 & -- & 121 (18.8\%) & 136 (21.2\%) & 206 (32.0\%) \\ \hline
%         \end{tabular}
%     }
%     \label{table:badcoinlist_2021}
% \end{table}

  

%Cluster 1 contains 81 crypto projects which have been poorly managed. Surprisingly, all crypto projects, which are included in Cluster 1, have not been updated for the last six months. The most representative examples in Cluster 1 are ReddCoin (RDD), Fastcoin (FST), TTC (TTC), Mooncoin (MOON), and Sumokoin(SUMO). In this cluster, 60 out of 82 (74.1\%) crypto projects have been recognized as inactive.\jusop{60 is N/A in CoinMarketCap + N/A in GitHub + Deadcoins + Coinopsy} Cluster 2 contains 207 crypto projects which have been poorly managed. Like Cluster 1, all crypto projects, which are included in Cluster 2, have not been updated for the last one year. The most representative examples in Cluster 2 are DigiByte (DGB), Lisk (LSK), Zcoin (XZC), LBRY Credits (LBC), and Gapcoin (GAP). In this cluster, 159 out of 207 (76.8\%) crypto projects have been recognized as inactive. Cluster 3 contains 243 crypto projects which are frequently updated. The most representative examples in Cluster 3 are Bitcoin (BTC), Ethereum (ETH), Ripple (XRP), Litecoin (LTC), and Cardano (ADA). In this cluster, 93 out of 243 (38.3\%) crypto projects have been recognized as inactive. Cluster 4 contains 61 crypto projects which are rarely updated during last 3 months. The most representative examples in Cluster 4 are NEM (XEM), Siacoin (SC), Prizm (PZM), Unobtanium (UNO), SaluS (SLS). In this cluster, 38 out of 61 (62.3\%) crypto projects have been recognized as inactive.

%\hljs{ in May 2020. In addition, 98 out of 355 (27.6\%) crypto projects have been recognized as inactive in May 2021. During 1 year, 19 crypto projects were additionally inactivated.} 

% \hljs{in May 2020. In addition, 178 out of 288 (61.8\%) crypto projects have been recognized as inactive in May 2021. During 1 year, 13 crypto projects were additionally inactivated.}

%From those results, we draw several conclusions. First, about half of crypto projects have been poorly maintained or abandoned -- 288 out of 643 (44.8\%) crypto projects have not been updated during the last six months. Second, it seems that the code update activities could be used to assess the survivability of projects -- the groups with frequently updated crypto projects (in Cluster 2) have the low proportion (22.3\%) of inactive projects. In contrast, the crypto projects in Cluster 1 that was rarely updated are highly like to be an inactive project (55.9\%). 

% \hljs{Third, there is no significant difference between clusters about the scam or inactive reports from CoinCodeCap, Deadcoins, and Coinopsy -- the groups with frequently updated crypto projects (in Cluster 2) are reported as the scam or inactive projects (43.1\% in May 2020 and 25.6\% in May 2021) . Similarly, the crypto projects in Cluster 1 that rarely updated are reported as the scam or inactive projects (62.9\% in May 2020 and 39.9\% in May 2021). However, the proportion of Cluster 1 is higher than the proportion of Cluster 2.} 
%Third, even though code maintenance activities can provide some valuable information about the survivability of projects, its applicability may also be limited in some instances. For example, our manual analysis shows that Uniform Fiscal Object, which was recognized as a project having negligible changes from the original Bitcoin code, is included in Cluster 2, which is a frequently updated group. This example shows the limitations of using code maintenance activity information alone.

\begin{comment}

\noindent \fbox{\begin{minipage}{\linewidth}
\hljs{Based on the clustering results, 355 (55.2 \%) crypto projects are frequently updated (\textbf{RQ1}). However, according to the example of Uniform Fiscal Object, updating information alone is not enough to determine which are poor projects.}
\end{minipage}}

\end{comment}

% \noindent \ovalbox{\begin{minipage}{\linewidth}
% \hljs{Based on the clustering results, 355 (55.2 \%) crypto projects are frequently updated (\textbf{RQ1}). However, according to the example of Uniform Fiscal Object, it is not enough to determine which one is the poor project using only updating information.}
% \end{minipage}}

\begin{comment}

We also tried to cluster the crypto projects with a single feature such as the number of commits for 3, 6, and 12 months. Because the clustering used a single feature, we used the ``kmeans1d'' library~\cite{kmeans1d}, a Python library with the implementation of $k$-means clustering on one-dimensional data, based on the algorithm in Xiaolin et al.~\cite{wu1991optimal}. As a result, every cluster using a single feature produced a bias cluster (639, 628, and 617 crypto projects clustered in the same cluster when we used the number of commits for 3, 6, and 12 months, respectively) in Table~\ref{table:single_feature3}, \ref{table:single_feature6}, and \ref{table:single_feature12}. Not surprisingly, most of the inactive projects are included in the massive cluster. Unlike the 3-month clustering, the 6-month and 12-month clustering sorted Bitcoin and Ethereum into different clusters.

\begin{table}[!ht]
    \centering
    \caption{Proportion of inactive crypto projects in each cluster in May 2020. Single feature (3 month).}
    \resizebox{0.95\linewidth}{!}{
    \begin{tabular}{|c|c|c|c|c|}
        \hline
        ID & \# & N/A in CoinMarketCap & N/A in GitHub & All \\\hline
        %Number (\%) & 103 (19.9\%) & 415 (80.1\%) & 231 (44.6\%) & 138 (26.6\%) & 25 (4.8\%) \\\hline
        1 & 639 & 227 (35.5\%) & 14 (2.2\%) & 239 (37.4\%) \\\hline
        2 & 4 & 1 (25.0\%) & 0 (0.0\%) & 1 (25.0\%) \\\hline
    \end{tabular}}
    \label{table:single_feature3}
\end{table}

\begin{table}[!ht]
    \centering
    \caption{Proportion of inactive crypto projects in each cluster in May 2020. Single feature (6 month).}
    \resizebox{0.95\linewidth}{!}{
    \begin{tabular}{|c|c|c|c|c|}
        \hline
        ID & \# & N/A in CoinMarketCap & N/A in GitHub & All \\\hline
        %Number (\%) & 103 (19.9\%) & 415 (80.1\%) & 231 (44.6\%) & 138 (26.6\%) & 25 (4.8\%) \\\hline
        1 & 628 & 225 (35.8\%) & 14 (2.2\%) & 237 (37.7\%) \\\hline
        2 & 15 & 3 (20.0\%) & 0 (1.7\%) & 3 (20.0\%) \\\hline
    \end{tabular}}
    \label{table:single_feature6}
\end{table}

\begin{table}[!ht]
    \centering
    \caption{Proportion of inactive crypto projects in each cluster in May 2020. Single feature (12 month).}
    \resizebox{0.95\linewidth}{!}{
    \begin{tabular}{|c|c|c|c|c|}
        \hline
        ID & \# & N/A in CoinMarketCap & N/A in GitHub & All \\\hline
        %Number (\%) & 103 (19.9\%) & 415 (80.1\%) & 231 (44.6\%) & 138 (26.6\%) & 25 (4.8\%) \\\hline
        1 & 617 & 224 (36.3\%) & 13 (2.1\%) & 235 (38.1\%) \\\hline
        2 & 26 & 4 (15.4\%) & 1 (3.9\%) & 5 (19.2\%) \\\hline
    \end{tabular}}
    \label{table:single_feature12}
\end{table}
\end{comment}



% To check whether 643 projects (collected in \hl{June} 2019) are still maintained well, we again collect the coin projects in the same manner that we initially used. The number of newly collected projects (in May 2020) is \hl{640} projects, where \hl{five} projects disappear, and \hl{two} projects are newly added. We found that 4 of 5 disappeared altcoins belong to either ``Cluster 1'' or ``Cluster 3''. Only one altcoin belongs to ``Cluster 4.'' The altcoins having low activities are much possible to disappear.

%To validate our observations in the survivability of crypto projects per cluster, we checked whether the 643 crypto projects (in September 2019) initially analyzed are still alive in May 2020 with the same criteria used in selecting those 643 crypto projects. That is, we regard a project as an alive one if the project is still registered on CoinMarketCap in May 2020, and its GitHub project URL is also still available. The survivability results are presented in Table~\ref{tab:disappear_coins}. We can see that a significant number of crypto projects (37.2\%) were excluded from CoinMarketCap or disappeared in GitHub in just 9 months. In particular, a majority of crypto projects in ``Cluster 1'' (51.5\%) and ``Cluster 3'' (50.0\%) disappeared. These findings are consistent with the results with the crypto projects reported as scam or inactive ones (see Table~\ref{table:badcoinlist}).

%50.2\%, 45.5\%, and 25.2\%, on the dropping out of CoinMarketCap list. On the other hand, the coins in ``Cluster 2'' have a few proportions (13.9\%) on the dropping out of CoinMarketCap list. As a result, 239 (37.2\%) of crypto projects have been disappeared during 2 years. In addition, the 79.9\% of the disappeared crypto projects are in ``Cluster 1'', ``Cluster 3'' and ``Cluster 4''. It means that the poor maintenance activity is directly related to the dead coins.

%\begin{table}[!ht]
%    \centering
%    \caption{Average on market information on May 2020. The unit capitalization column is millions.}
%    \resizebox{0.99\linewidth}{!}{
%    \begin{tabular}{|c|c|c|c|c|c|c|}
%        \hline
%        \multirow{2}{*}{Cluster ID} & \multicolumn{2}{c|}{Ranking} & \multicolumn{2}{c|}{Market capitalization} & \multicolumn{2}{c|}{Price} \\ \cline{2-7} 
%         & ave. (diff.) & std. & ave. (diff.) & std. & ave. (diff.) & std. \\\hline
%        1 & 1334.4 (+459.7) & 737.1 & 23M (-64M) & 138M & 0.1 (-0.6) & 0.6 \\\hline
%        2 & 515.1 (+63.8) & 434.2 & 840M (-1,003M) & 4,188M & 11.1 (-17.3) & 39.5 \\\hline
%        3 & 1477.0 (+587.5) & 584.1 & 3M (-4M) & 11M & 0.0 (-0.2) & 0.1 \\\hline
%        4 & 1037.9 (+407.9) & 646.0 & 21M (-48M)& 87M & 0.4 (-1.5) & 1.9 \\\hline
%        5 & 839.0 (+343.9) & 661.9 & 6,970M (+1,578M) & 34,085M & 1262.7 (+95.1) & 5145.8 \\\hline
%        6 & 1212.6 (+489.4) & 632.7 & 16M (-44M) & 59M & 1.6 (-3.4) & 8.2 \\\hline
%        7 & 778.9 (+229.3) & 642.5 & 211M (-315M) & 1,135M & 0.5 (-2.4) & 2.5 \\\hline
%        All &              &       &              &        &            &     \\\hline
%    \end{tabular}}
%    \label{tab:market_info_2020}
%\end{table}

==> Coin code similarity (Version 51646)/sec/results_originality.tex <==
\section{Code similarity analysis}
\label{sec:results_originality}

This section presents the results of the source code similarity analysis between crypto projects using the method described in Section~\ref{subsec:originality_method}. 

%We specifically identify Bitcoin's descendent cryptocurrencies and analyze how much those descendent cryptocurrencies have been updated over time after forking.

%This section presents the results of the source code similarity analysis between crypto projects using the method described in Section~\ref{subsec:originality_method}. First, we calculate the similarity scores between C-based crypto projects with their latest version. With the similarity score results, we can see that there are several clusters of crypto projects in terms of code similarity. Next, we specifically identify Bitcoin's descendent cryptocurrencies and analyze how much those descendent cryptocurrencies have been updated over time after forking. Finally, we examine 20 altcoins that are highly similar to the version of Bitcoin used for the fork and uncover 9 of them which do not contain any technically-meaningful changes from Bitcoin, without the implementation of features mentioned in their whitepapers.

\begin{comment}

\subsection{Analysis of similarity between C-based crypto projects}
\label{subsec:traditionalsimilarity}

We calculated the similarity scores for $\binom{511}{2} = 130,305$ pairs of C-based crypto projects using the \texttt{JPlag}-based repository-to-repository comparison method~\cite{jplag} described in Section~\ref{subsec:originality_method}. 

\begin{figure}[!ht]
\vspace{-0.2cm}
\centering
\includegraphics[width=0.7\columnwidth,clip]{fig/c_heatmap_subfigure.png}
\vspace{-0.2cm}
\caption{Heatmap showing the similarity scores between XXX C-based cryptocurrencies.}
\label{fig:totalheatmap}
\end{figure}

%The heatmap shows that there is only a small proportion of white lines representing crypto projects that are completely unique from other projects.

Fig.~\ref{fig:totalheatmap} shows the heatmap of code similarity scores of pairwise comparisons for C-based crypto projects. In the heatmap, darker colors correspond to higher similarity scores -- the highest similarity scores are found for the same cryptocurrency comparisons across the diagonal axis with several clusters. The heatmap shows that most crypto projects can be clustered into a small number of subgroups in terms of code similarity. %\hljs{Appendix}~\ref{appendix:CDF_latest_latest} \hljs{shows the CDF of the similarity scores between C-based crypto projects.}

Fig.~\ref{fig:cdf_latest_latest} shows the cumulative distribution function (CDF) of the similarity scores between C-based crypto projects. Among 130,305 pairs of those projects, 1.7\% of the pairs have 95\% or more code similarity; 3.5\% of the pairs have 90\% or more; 10.4\% of the pairs have 80\% or more; 30.4\% of the pairs have 60\% or more; and 43.6\% of the pairs have 50\% or more. 

\begin{figure}[!h]
\centering
\includegraphics[width=0.7\columnwidth]{fig/CDF_latest_latest.pdf}
\vspace{-0.1cm}
\caption{Cumulative distributions function (CDF) of the similarity scores between 511 C-based cryptocurrencies.}
\label{fig:cdf_latest_latest}
\end{figure}

With the similarity scores, we grouped C-based crypto projects into clusters using the affinity propagation clustering algorithm~\cite{frey2007clustering} to identify groups of similar crypto projects at the code level. The results of this algorithm are a set of clusters containing similar crypto projects. The clustering results for C-based cryptocurrencies are presented in Appendix~\ref{appendix:Code similarity-based clustering results}. In the clustering result, the number of clusters is XX, and the largest cluster included XX projects. Bitcoin is contained in Cluster 6 with XX crypto projects, which have the mean similarity score of XX.X\% with the standard deviation of XX.X\%.

\end{comment}

\subsection{Analysis of similarity between altcoins and Bitcoin}
\label{subsec:newmethodsimilarity}

To investigate whether altcoins have made significant enhancements from their original parent project, we specifically focused on Bitcoin and its descendent cryptocurrencies because many altcoins were advertised as addressing various limitations of Bitcoin. This analysis is therefore crucial to evaluating not just the maintainability of crypto projects but also their justification and the truthfulness or otherwise of the claims used to market them. As living software should be continuously updated to add new features or fix bugs, projects that are not being maintained may have been quietly abandoned.

We used the heuristic methods described in Section~\ref{subsec:originality_method} to identify those crypto projects and estimate their forking times. When Heuristic 2 is used, we specifically set the similarity threshold to 92.9\% to determine whether a project is forked or not. This threshold was obtained by the mean similarity score (99.4\%) between Bitcoin and its altcoins minus three standard deviations (6.5\%), obtained from the Heuristic 1 method, based on the three-sigma limits. In Heuristic 2, if the similarity score between an altcoin and the version of Bitcoin used while creating the fork is greater than 92.9\%, we assumed that the altcoin was forked from Bitcoin even though the altcoin was not explicitly forked through GitHub. From 510 C-based crypto projects, we found that 157 altcoins are likely to have been forked from Bitcoin. Among those projects, we confirm that 154 projects have entered the mainnet; one project is still in the testnet phase; we cannot determine the status of the remaining two. 127 altcoins were discovered by Heuristic 1, while 30 altcoins were discovered by Heuristic 2. Table~\ref{table:altcoin_disappear} shows the proportion of those projects with their similarity scores, revealing that about a third of the 157 altcoins that are likely to have been forked from Bitcoin still have 90\% or more code similarity with the Bitcoin version used to spawn them. 

\begin{table}[t]
\vspace{-0.3cm}
\centering
\caption{Proportion of inactive/scam crypto projects with the similarity scores.}
\label{table:altcoin_disappear}
\resizebox{0.85\linewidth}{!}{
\begin{tabular}{|c|r|r|r|r|r|r|}
\hline
Similarity score & \multicolumn{1}{c|}{Number (\%)} & \multicolumn{1}{c|}{N/A in CoinMarketCap} & \multicolumn{1}{c|}{N/A in GitHub} & \multicolumn{1}{c|}{Coinopsy} & \multicolumn{1}{c|}{Deadcoins} & \multicolumn{1}{c|}{All} \\\hline
$\geq 95\%$ & 34 (21.7\%) & 16 (47.1\%) & 0 (0.0\%) & 12 (35.3\%) & 11 (32.4\%) & 24 (70.6\%) \\\hline
$\geq 90\%$ & 53 (33.8\%) & 25 (47.2\%) & 0 (0.0\%) & 17 (32.1\%) & 17 (32.1\%) & 38 (71.7\%) \\\hline
$\geq 80\%$ & 66 (42.0\%) & 31 (47.0\%) & 1 (1.5\%) & 19 (28.8\%) & 17 (25.8\%) & 46 (69.7\%) \\\hline
$\geq 60\%$ & 95 (60.5\%) & 36 (37.9\%) & 1 (1.1\%) & 24 (25.3\%) & 22 (23.2\%) & 57 (60.0\%) \\\hline
%$\geq 50\%$ & 114 & 42 (36.8\%) & 3 (2.6\%) & 26 (22.8\%) & 24 (21.1\%) & 64 (56.1\%)\\\hline
$<50\%$     & 43 (27.4\%) & 11 (25.6\%) & 1 (2.3\%) & 10 (23.3\%) & 5 (11.6\%) & 18 (41.9\%) \\\hline
All         & 157 (100.0\%) & 52 (33.8\%) & 4 (2.5\%) & 36 (22.9\%) & 29 (18.5\%) & 82 (52.2\%) \\\hline
\end{tabular}}
\vspace{-0.6cm}
\end{table}

\begin{comment}

The estimated fork times of those projects can be shown in Fig.~\ref{fig:forkingpointgraph}. Among the forked projects, the oldest one is HunterCoin, forked in July 2011, while the latest one is FujiCoin, forked in March 2019.

\begin{figure}[!h]
\centering
\includegraphics[scale=0.2]{fig/ForkingPointGraph.pdf}
\vspace{-0.1cm}
\caption{Histogram of estimated forking times for altcoins.}
\label{fig:forkingpointgraph}
\end{figure}
\end{comment}

To verify the correctness of the forked projects identified by our heuristic methods, we compare those projects with a list of known Bitcoin descendants (\url{https://mapofcoins.com/bitcoin/}). From the 175 cryptocurrencies active in December 2017, we selected 68 included in our dataset for testing (hereinafter referred to as the ``known list''). Most of the remaining ones were defunct when we started collecting data on July 22nd, 2018. For a fair comparison, among the 157 cryptocurrencies identified as forked projects by our method, we also considered 139 (hereinafter referred to as ``our list'') that were forked before December 2017. By comparing ``our list'' against the ``known list,'' we observed only 33 cryptocurrencies in both lists. That is, our method was able to identify additional 106 coins whose Bitcoin ancestry was not included in the ``known list.'' However, our method failed to infer the forking relationships of the 35 remaining coins in that list. We manually checked these failure cases and found that those altcoins were created by externally uploading an old version of Bitcoin as new files to a repository. Although Heuristic 2 is designed to detect such cases, Heuristic 2 can also suffer false negatives because, for performance reasons, it does not examine all previous versions of Bitcoin. This limitation is discussed in Section~\ref{sec:limit}.
%A majority of the cryptocurrencies were forked in 2014 Q2 (18.9\%), 2011 Q3 (15.1\%), and 2017 Q3 (9.4\%).

%We note that 128 altcoins discovered by Heuristic 1 were clearly forked from Bitcoin because their commit history is the same as that of Bitcoin, which can only be observed in forked repositories. However, for the 31 altcoins discovered by Heuristic 2, we cannot check their explicit forking information. 

%Our goal is to examine whether those forked projects have been sufficiently modified from Bitcoin to justify their establishment as separate blockchain products. To that end, we measured the similarity between the forked projects and Bitcoin.

Fig.~\ref{fig:difference_c} shows the CDF (dashed blue line) of the similarity scores between Bitcoin and its descendent cryptocurrencies. Only 6 out of 157 (3.8\%) crypto projects forked from Bitcoin have 90\% or more code similarity with the latest version of Bitcoin. From these findings, however, we cannot conclude how much altcoins have changed over time because Bitcoin itself changes significantly. Therefore, to examine how much a forked altcoin has changed from Bitcoin, we compute the similarity score between the latest source code of the forked project and the source code of Bitcoin at the time of the fork. Fig.~\ref{fig:difference_c} shows the CDF (solid red line) of the similarity scores between them. Among 157 projects forked from Bitcoin, 21.7\% of the pairs have 95\% or more code similarity; 33.8\% of the pairs have 90\% or more; 42.0\% of the pairs have 80\% or more; and 60.5\% of the pairs have 60\% or more. These results confirm that forked projects are most similar to their parent version of Bitcoin. This finding implies that a significant number of forked projects contain only negligible changes from the parent version of Bitcoin at the time of the fork.

%; and 72.6\% of the pairs have 50\% or more

\begin{figure}[t]
\vspace{-0.1cm}
\centering
\includegraphics[width=0.58\linewidth]{fig/CDF_pastcurrent_currentcurrent.pdf}
\vspace{-0.2cm}
\caption{CDFs of the similarity scores between altcoins and Bitcoin (Latest: similarity scores between the latest version of altcoins and the latest version of Bitcoin, Forked: similarity scores between the latest version of altcoins and the version of Bitcoin used for the fork).}
\label{fig:difference_c}
\vspace{-0.6cm}
\end{figure}

\begin{comment}
Bitcoin is continuously being updated. To confirm this, we analyzed how much the source code of Bitcoin has changed from June 2014 until September 2019. Fig.~\ref{fig:btchistory} shows the similarity scores, comparing the latest version (September 2019) of Bitcoin against all previous versions, starting from June 2014. Bitcoin changed significantly in the past five years. Compared to the latest version, the June 2014 version shows only 34.1\% similarity. The similarity score for Bitcoin version comparisons tends to increase linearly over time. 

\begin{figure}[!h]
\centering
\includegraphics[width=0.7\linewidth]{fig/btc_eth_history.pdf}
\vspace{-0.2cm}
\caption{Similarity scores with the latest version (September 2019) of Bitcoin for all the previous versions of Bitcoin from June 2014 to September 2019.}
\label{fig:btchistory}
\end{figure}
\end{comment}

%(see Appendix~\ref{appendix:bitcoin_history}).

%, while the November 2015 version shows about 50\%





% >= 95, T: 34, D: 18, E: 16
% 95 > ~ >= 90, T: 21, D: 10, E: 11
% 90 > ~ >= 80, T: 13, D: 5, E: 8
% 80 > ~ >= 60, T: 29, D: 7, E: 22
% 60 > ~ >= 50, T: 19, D: 5, E: 14
% 50 >, T: 43, D: 7, E: 36

%We regard a project as an active one if the project is still registered on CoinMarketCap in May 2020, and its GitHub project URL is also still available. 

% \footnote{\hljs{We defined the word ``survivability'' as the delisted crypto project from CoinMarketCap. However, note that the delisted does not mean the scams. Feder et al.}~\cite{feder2018rise} \hljs{shows that a delisted altcoin could return.}}

To show the relevance of code similarity, we analyzed the relationship between the survivability of the projects forked from Bitcoin and their similarity scores. As presented in Table~\ref{table:altcoin_disappear}, the projects with high similarity scores are likely to disappear from the market or be reported as a scam or inactive: 70.6\% of altcoins with 95\% or more code similarity suffered this fate, compared with only 41.9\% of altcoins with similarity scores less than 50\%.


%To analyze the survivability of those altcoins with similarity scores, we checked whether they are still alive in May 2020 in the manner described in Section~\ref{sec:results_maintenance}. We note that a third of them have been recognized as inactive. The survivability results are presented in Table~\ref{table:altcoin_disappear}. The scores could be used to predict project survivability. 52.9\% of altcoins having 95\% or more code similarity were delisted from CoinMarketCap, while only 16.3\% of altcoins having similarity scores less than 50\% were delisted.

%\vspace{-0.4cm}

\subsection{Case studies}
\label{subsec:Case studies}

To identify altcoins that did not implement the unique features claimed in their whitepapers, we examined source code and whitepaper contents for the top 20 altcoins with the highest similarity scores with their parent version of Bitcoin (see Appendix~\ref{appendix:Top 20 altcoins that are highly similar to the version of Bitcoin used for the fork}).

%(see Appendix~\ref{appendix:Top 20 altcoins that are highly similar to the version of Bitcoin used for the fork}).%The top 20 altcoins that are highly similar to the version of Bitcoin used for the fork %Appendix~\ref{appendix:Top 20 altcoins that are highly similar to the version of Bitcoin used for the fork} shows the top 20 altcoins that are highly similar to the version of Bitcoin used for the fork. %Interestingly, 10 (50\%) out of the 20 altcoins are inside Cluster 1 (see clustering results in Section~\ref{sec:results_maintenance}).

%BetaCoin (BET), Fujicoin (FJC), 

%We manually investigated the commits and source code of all the 20 altcoins. 

Among those altcoins, MinCoin (MNC), GapCoin (GAP), Litecoin (LTC)\footnote{Although Litecoin was initially forked from Bitcoin on October 13th, 2011, the old project was deprecated, and a new Litecoin project was created again by forking from the ``August 13th, 2018'' version of Bitcoin.}, Platincoin (PLC), Florincoin (FLO), MinexCoin (MNX), Riecoin (RIC), Fujicoin (FJC), Feathercoin (FTC), Octocoin (888), and Uniform Fiscal Object (UFO) are variants of Bitcoin that made slight modifications in the way cryptographic algorithms are used for proof of work, and in policy parameter values (e.g., total supply, block generation time). Uniform Fiscal Object has been frequently updated -- every 0.1 days on average. This project has been clustered into Cluster 4, consisting of frequently updated projects. However, most commits we inspected contain changes in comments, icons, genesis block, and total supply. We found the only meaningful change was the replacement of SHA-256 with NeoScrypt in the hash function used for mining.

We found that the remaining nine crypto projects do not contain any technically meaningful code change. The most frequent changes were cryptocurrency name changes. For example, Acoin (\url{https://aco.ample-cosplay.com/}) is a copycat of Bitcoin that did not add any noticeable new feature after the fork. The only changes we noticed were replacing ``bitcoin'' with ``acoin'' in some code fragments (see Fig.~\ref{fig:code_example}). 

%according to the white paper (\url{http://freico.in/docs/freimarkets.pdf}), Freicoin was designed to provide a method that converts rights to assets into digital tokens on a blockchain. However, we found that most commits were related to changing crypto names (e.g., replacing ``bitcoin'' to ``freicoin''), and to modifying blockchain policies (see Figure~\ref{fig:code_example}). The last commit of Freicoin was on October 8th 2018.

\begin{figure}[!ht]
\vspace{-0.2cm}
\centering
\includegraphics[width=0.99\linewidth]{fig/code_example.png}
\vspace{-0.3cm}
\caption{A change in the ``miner.cpp'' file in Acoin.}
\label{fig:code_example}
\vspace{-0.4cm}
\end{figure}

More worryingly, six crypto projects did not appropriately implement features promised in their whitepapers. For example, according to the whitepaper (\url{http://bit.ly/blockarray-whitepaper}) written for Block Array (ARY), it was designed to facilitate the development of protocols for logistics. The whitepaper also presented a timeline and road map until 2020. However, we found just two commits for Block Array: the first was about uploading the Bitcoin project files, and the second, on December 29th, 2017, created the \texttt{README.md} file. Although Block Array reused the entire Bitcoin source code, the whitepaper does not explain this. Its official website (\url{https://www.blockarray.com/}) does not even exist. 

%and supply chain management






%Florin (FLO) is also a slightly modified version of Bitcoin, which adds the support for adding transaction comments to coin transactions. 

%Worryingly, projects like Freicoin, PLNcoin, CHIPS, Octocoin, Carboncoin, CHANCOIN, and Internet of People seem no longer active or have already been reported as scams.



% Freicoin (FRC): Deadcoins, Coinopsy
% PLN: Coinopsy
% CARBON: CoinCodeCap
% Octocoin: Coinopsy





%BetaCoin (BET) was designed to provide faster transaction confirmation by changing some parameter values such as mining difficulty and total supply. However, we can find a commit (\url{https://github.com/BetaCoinDev/betacoin/commit/6750f32ca106307e52287e5b8092e8cc2413514c}) of the code update about \texttt{MAX\_MONEY}. The last commit of BetaCoin (BET) was made on April 3rd 2014, and most commits were related to fixing some Bitcoin vulnerabilities and modifying policy parameter values. However, their updated codes do not actually change the Bitcoin's policies. Its official website (\url{https://betacoin.info/}) does not exist.

There were seven projects for which the official websites have disappeared. For example, PLNcoin's (PLNC) official website URL (\url{https://plncoin.org/}) has been redirected to a suspicious website. CHIPS' Git repository only contains the link of the official Bitcoin Core website. %Octocoin's official website (\url{http://octocoinfoundation.org/}) does not work.

% Interestingly, \hljs{CHIPS (CHIPS) has been updated every 45.5 days on average. Therefore, this project has been clustered into Cluster 2, which consists of frequently updated projects. However, most commits we inspected contain changes in comments, icons, genesis blocks, and the total number of blocks. We cannot find any significant changes between Bitcoin and CHIPS in algorithms, data structures, and protocols except the replacement of SHA-256 with NeoScrypt in the hash function for the mining process.}

%Similarly, the following crypto projects contain only negligible changes from the parent Bitcoin project, and do not implement features promised in their white papers. The last commits of Acoin (ACOIN), C-Bit (XCT), DeusCoin (DEUS), and BlueCoin (BLU) were on October 23rd 2014, September 4th 2017, November 15th 2017, and October 2nd 2017.  The last commit of PLNcoin was on February 12th 2018, where its official website domain name (\url{https://plncoin.org/}) has been redirected to a suspicious website. The last commit of CHIPS was on October 9th 2018, and its GitHub repository contains only the link of the official Bitcoin Core website. The last commit of Octocoin was on April 18th 2016, and most links on its official website (\url{http://octocoinfoundation.org/}) have been broken. Interestingly, Uniform Fiscal Object (UFO) has been frequently updated every 0.1 days on average. Therefore, this project has been clustered into Cluster 2, which consists of frequently updated projects. However, most commits we inspected contain changes in comments, icons, genesis blocks, and the total number of blocks. We cannot find any significant changes between Bitcoin and Uniform Fiscal Object in algorithms, data structures, and protocols.

%SecureCoin has only two commits and its last commit was made on August 28th 2013.

%Interestingly, Internet of People has been updated every 3.1 days on average. Therefore, this project has been clustered into ``Cluster 2,'' which consists of frequently updated projects, and has not been registered as a scam. However, most commits we inspected contain changes in comments, icons, and names (e.g., replacing ``BTC'' with ``IOP''). There was only one notable modification by allowing only whitelisted nodes to participate in the proof-of-work consensus process. We cannot find any significant changes between Bitcoin and Internet of People in algorithms, data structures, and protocols.

Finally, sixteen projects disappeared from the market, or were reported as scams or inactive by September 2021. Half of them have already been reported as scam coins: GapCoin, Freicoin, PLNcoin, MinexCoin, Riecoin, SecureCoin, and OctoCoin were flagged as scams in Coinopsy~\cite{coinopsy}, while Betacoin, Freicoin, PLNcoin, MinexCoin, Riecoin, FujiCoin, SecureCoin, and Uniform Fiscal Object were flagged as scams in Deadcoins~\cite{deadcoins}. Our findings indicate that code-similarity metrics might provide a better signal to detect inactive or scam projects than such public reporting services. 

%CoinCodeCap~\cite{coincodecap} flagged MinCoin as a scam.

\begin{comment}

\noindent \fbox{\begin{minipage}{\linewidth}
\hljs{Among 159 Bitcoin-based altcoins, 73\% of the pairs have 50\% or more code similarity. In other words, many crypto projects forked from Bitcoin aren't making significant code changes (\textbf{RQ3}).}
\end{minipage}}

\end{comment}

==> Makefile <==
#
# Makefile for acmart package
#
# This file is in public domain
#
# $Id: Makefile,v 1.10 2016/04/14 21:55:57 boris Exp $
#

PACKAGE=acmart


PDF = $(PACKAGE).pdf acmguide.pdf

all:  ${PDF} ALLSAMPLES


%.pdf:  %.dtx   $(PACKAGE).cls
	pdflatex $<
	- bibtex $*
	pdflatex $<
	- makeindex -s gind.ist -o $*.ind $*.idx
	- makeindex -s gglo.ist -o $*.gls $*.glo
	pdflatex $<
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $*.log) \
	do pdflatex $<; done


acmguide.pdf: $(PACKAGE).dtx $(PACKAGE).cls
	pdflatex -jobname acmguide $(PACKAGE).dtx
	- bibtex acmguide
	pdflatex -jobname acmguide $(PACKAGE).dtx
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' acmguide.log) \
	do pdflatex -jobname acmguide $(PACKAGE).dtx; done

%.cls:   %.ins %.dtx
	pdflatex $<


ALLSAMPLES:
	cd samples; pdflatex samples.ins; cd ..
	for texfile in samples/*.tex; do \
		pdffile=$${texfile%.tex}.pdf; \
		${MAKE} $$pdffile; \
	done

samples/%: %
	cp $^ samples


samples/$(PACKAGE).cls: $(PACKAGE).cls
samples/ACM-Reference-Format.bst: ACM-Reference-Format.bst

samples/%.pdf:  samples/%.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex-dev $(notdir $<); done

samples/sample-xelatex.pdf:  samples/sample-xelatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && xelatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && xelatex-dev $(notdir $<)
	cd $(dir $@) && xelatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && xelatex-dev $(notdir $<); done

samples/sample-lualatex.pdf:  samples/sample-lualatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && lualatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && lualatex-dev $(notdir $<)
	cd $(dir $@) && lualatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && lualatex-dev $(notdir $<); done



.PRECIOUS:  $(PACKAGE).cfg $(PACKAGE).cls

docclean:
	$(RM)  *.log *.aux \
	*.cfg *.glo *.idx *.toc \
	*.ilg *.ind *.out *.lof \
	*.lot *.bbl *.blg *.gls *.cut *.hd \
	*.dvi *.ps *.thm *.tgz *.zip *.rpi \
	samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst \
	samples/*.log samples/*.aux samples/*.out \
	samples/*.bbl samples/*.blg samples/*.cut 



clean: docclean
	$(RM)  $(PACKAGE).cls \
	samples/*.tex

distclean: clean
	$(RM)  *.pdf samples/sample-*.pdf

#
# Archive for the distribution. Includes typeset documentation
#
archive:  all clean
	COPYFILE_DISABLE=1 tar -C .. -czvf ../$(PACKAGE).tgz --exclude '*~' --exclude '*.tgz' --exclude '*.zip'  --exclude CVS --exclude '.git*' $(PACKAGE); mv ../$(PACKAGE).tgz .

zip:  all clean
	zip -r  $(PACKAGE).zip * -x '*~' -x '*.tgz' -x '*.zip' -x CVS -x 'CVS/*'

documents.zip: all docclean
	zip -r $@ acmart.pdf acmguide.pdf samples *.cls ACM-Reference-Format.*

.PHONY: all ALLSAMPLES docclean clean distclean archive zip


==> sec/research_question.tex <==
\section{Research questions}
\label{sec:research_questions}
%This paper has been motivated by the following three research questions. %\hljs{This paper has been motivated by evaluating the crypto projects ecosystem with the following three research questions.}

The market for altcoins appears to be a classic ``market for lemons''~\cite{Akerlof70:lemon} in that investors lack information about crypto projects' code originality, maintenance, and security, and have to rely on marketing material such as whitepapers on project websites. There is little motivation for companies to implement promised features honestly or quickly patch security vulnerabilities since investors have no easy way of checking their development activities or verifying whether updates claimed on websites or social media are indeed being committed to code repositories. This paper aims to facilitate the identification of potential \emph{crypto lemons} in the market -- projects that are unoriginal, vulnerable, or both -- to help investors assess financial and security risks better. We focus on the following three research questions to achieve this goal:

%\textbf{RQ1: \hl{How many crypto projects have persistently been maintained in source code?}}

\textbf{RQ1: Are crypto projects updating their source code?}

One way to assess the liveness and credibility of a crypto project is to investigate its code maintenance activities. To answer RQ1, we designed an evaluation framework that automatically analyzes a project's source code and commits to its code repository.

%\textbf{\hl{RQ2: How many crypto projects have  been updated for security patches in a timely manner?}}

\textbf{RQ2: Are crypto projects implementing security patches in a timely manner?}

To evaluate the security of crypto projects, we analyze how quickly known security vulnerabilities have been patched. To answer RQ2, we identify vulnerable code fragments in crypto projects and investigate when these code fragments were patched. According to Gartner's report~\cite{gartner}, about 90\% of successful Internet-based attacks that exploited software applications have not been patched properly. Therefore, if a crypto project ignores vulnerabilities or patches slowly, this indicates high-security risks.

\textbf{RQ3: Are crypto projects forked from Bitcoin making significant code changes to the original code?}

%More than 2,000 different altcoins have been launched since July 2011 to address inadequacies (e.g., transaction throughput, latency, or anonymity) in existing cryptocurrencies such as Bitcoin. 

To answer RQ3, we investigate whether these altcoins have indeed made meaningful enhancements from their original parent projects (e.g., by implementing the features promised in their whitepapers). We do not claim that the code similarity measurement alone is sufficient to identify scam or inactive projects. However, the code similarity measurement examines whether forked projects have been sufficiently modified from the original Bitcoin code over time to justify their establishment as a new blockchain product. 

%For this analysis, we focus on Bitcoin-forked projects, as Bitcoin is the most widely adopted cryptocurrency and has the biggest market capitalization.


